SoK: Access Control Policy Generation from High-level Natural Language Requirements

Administrator-centered access control failures can cause data breaches, putting organizations at risk of financial loss and reputation damage. Existing graphical policy configuration tools and automated policy generation frameworks attempt to help administrators configure and generate access control policies by avoiding such failures. However, graphical policy configuration tools are prone to human errors, making them unusable. On the other hand, automated policy generation frameworks are prone to erroneous predictions, making them unreliable. Therefore, to find ways to improve their usability and reliability, we conducted a Systematic Literature Review analyzing 49 publications, to identify those tools, frameworks, and their limitations. Identifying those limitations will help develop effective access control policy generation solutions while avoiding access control failures.

==> Sections/access_control.tex <==
\section{Access Control}
\label{sec:access_control}

% In this section, we introduce some popular access control models.
% % background on 2 concepts that the SLR is based on, namely access control and natural language processing. 

% \subsection{Access Control}

Access control in cybersecurity is a technique that regulates the authorization of users to perform a particular action on a resource in a computer system. In order to control access in a system with different levels of granularity and maintainability, several access control models have been proposed. Therefore, in this section, we introduce some of the key access control models that are widely used in the included publications of this SLR. 

\subsubsection{Access Control List (ACL)}

ACL is the low-level representation of the access control policies, which is organized as an ordered list \cite{nobi2022machine}. ACL typically connects an object with a list of users and groups. An operation can be performed on a resource by the user only if the operation and the user or the group that the user belongs to are mentioned in the list associated with the object \cite{barkley1997comparing}. 
% For instance, ACL for a file object can be defined as, 
% \begin{verbatim}
%     (Alice: read, write; Bob: read)
% \end{verbatim}
% According to the above ACL, Alice can read and write to the file object while Bob is allowed only to read the file object. Often ACLs are considered to be difficult to manage, as each user and the object is managed separately \cite{nobi2022machine}.

% \subsubsection{Discretionary Access Control (DAC)}

% DAC allows the administrators complete control of any object they own with the actions that are associated with the object. In contrast to ACLs, DAC restricts access to objects based on the user's identity and can be implemented using ACLs or Capabilities \cite{sandhu1994access}. Because of the less restrictive nature of DAC, on the one hand, there is a possibility that users have higher privileges than they are supposed to. On the other hand, the privileges of users are inherited to the programs that they execute.

% \subsubsection{Mandatory Access Control (MAC)}

% MAC is an access control model which allows the administrator to take access control decisions based on the security labels of the subject (clearance) and the object (sensitivity) \cite{sandhu1994access, sandhu1993lattice}. In contrast to DAC, any user except the administrator has no control over the access control policy configurations. There are 2 security models within MAC, namely Biba \cite{biba1977integrity} (utilized in businesses) and Bell-LaPadula \cite{bell1973secure} (utilized in military applications). Biba model focuses on the integrity of the information while the Bell-LaPadula model focuses on confidentiality. Further, there are 2 principles in Biba namely \emph{Read-up} which allows the users with lower clearance to read information with higher clearance, and \emph{Write-down} which allows the users with higher clearance to write for lower levels of clearance. On the other hand, the Bell-LaPadula model also has 2 principles. \emph{Read-down} which allows the users from higher levels to read lower-level information and to write for higher levels (\emph{Write-up}). 

\subsubsection{Role-based Access Control (RBAC)}

In RBAC, access will be granted/ denied based on the role of the user in the organization. Instead of assigning permission to every single user, the administrator will define roles with required permissions to assign users to the roles. Roles will be decided based on the actions and responsibilities associated with a particular organizational role \cite{sandhu1994access}. Further, a user can have multiple roles as well as a role can have multiple users. The same relation applies to user permissions and role permissions \cite{sun2022hybrid}. Furthermore, it is worth noting that, RBAC offers dynamic, static, and historic separation of duties (SoD) while allowing the administrator to define other constraints such as least privilege, mutually exclusive roles, and cordiality constraints \cite{nobi2022machine, ahn2010representing, sun2022hybrid}. There are several derivations of the RBAC model that also can be found in literature such as P-RBAC which extends RBAC with support for privacy policies \cite{vaniea2008access}.
% Even though RBAC was introduced as an alternative to DAC and MAC \cite{ahn2010representing}, the maintainability was vastly improved \cite{sandhu1994access}. For instance, if the responsibilities of a user change, the administrator only needs to assign the user to the new role. If the authorization is directly between the user and the objects, it is necessary to revoke all the access rights and assign new rights to new objects. 

\subsubsection{Attribute-based Access Control (ABAC)}
Due to the inadequacy of the aforementioned access control models to cope with the increasing complexity of the present business environment, ABAC was introduced \cite{alohaly2018deep}. Therefore, ABAC is often introduced as a more granular form of RBAC. NIST (National Institute of Standards and Technology) defines ABAC as ``An access control method where subject requests to perform operations on objects are granted or denied based on assigned attributes of the subject, assigned attributes of
the object..."\cite{hu2013guide}. According to the aforementioned definition, ABAC policy often contains several types of attributes including user attributes, resource attributes, and environmental conditions \cite{nobi2022machine}. A user will be authorized to access a resource by checking the above attributes in the access control request against the attributes in the policy. Despite having a promising potential, manual development of ABAC policy is considered costly since it involves some laborious processes such as attribute engineering, attributes assignment to the user and objects, policy engineering, etc \cite{hu2013guide, nobi2022machine, narouei2017towards}. 

% \subsection{Policy Languages}

% After extracting the policy components from a natural language access control policy, they should be combined into a machine executable format using a structured policy language. According to Anderson \cite{anderson2006comparison}, there are several requirements that a structured privacy policy language should satisfy in order to support expressions and enforcement of policies. 
% \begin{enumerate}
%     \item Language must support constraints on who is allowed to perform which action on which resources as well as it must support matching the purposes of accessing the particular resources.
%     \item The language must enable the expression of directly-enforceable policies.
%     \item Language must be platform independent.
% \end{enumerate}
% In this section we introduce one of the popular policy languages that agree with aforementioned requirements.

% \subsubsection{eXtensible Access Control Markup  Language (XACML)}

% XACML is based on the abstract model for policy enforcement defined by the IETF \cite{yavatkar2000framework}. In this model all requests that intend to access a protected resource should go through a Policy Enforcement Point (PEP). PEP formulates the request for an authorization decision with a description of the access request including its subject, resource, operation, purpose and other relevant information \cite{anderson2006comparison}. Then the authorization decision request will go through Policy Decision Point (PDP). PDP first extracts the policies applicable to the request with any additional information required to evaluate those policies retrieved from PIP (Policy Information Point). Then it evaluates the policies and returns the authorisation decision back to PEP. In XACML, policy authorisation decision would be one of  ``allow access", ``deny access", or ``no policies apply to this access request". If the PDP cannot evaluate the policies, it will return an error. Based on the decision, PEP will grant or deny the access which was requested. As additional information, the decision may contain obligations which are actions the PEP must take in conjunction  with  enforcing  the  authorization  decision. 

% There are 3 main top level elements in a XACML policy. $<Rule>$ is the basic unit of a XACML policy, containing a boolean expression that can be evaluated in separately. $<Policy>$ contains multiple $<Rule>$ elements and a specified procedure for combining the outcome of each $<Rule>$. As some of the rule combining algorithms, ``deny-overrides", ``permit-overrides", and ``first-applicable" can be mentioned. Finally, $<PolicySet>$ contains one or more $<Policy>$ or $<PolicySet>$ components with a specified procedure to evaluate the outcomes of child components. Every element mentioned above contains the $<Target>$ element which specifies the attributes to match with the access request. 



==> Sections/methodology.tex <==
\section{Planning and Conducting the SLR}
\label{sec:slr}

In order to identify the previous attempts on developing tools/ techniques to generate access control policies, we conducted a Systematic Literature Review (SLR) via a scientific and reproducible approach. SLR is a \emph{secondary study} which consists of 2 main stages: planning the review and conducting the review \cite{kitchenham2004procedures}. Therefore, in this section, we describe the above 2 stages according to our area of interest. 

\subsection{Planning the review}
\label{subsec:planning}

Planning the SLR is mainly about identifying the need for the review and developing a review protocol to avoid research bias \cite{kitchenham2004procedures}. With that in mind, we conducted the following activities under this section. 

\begin{enumerate}
    \item Defining the research scope
    \item Formulation of the research questions that need to be answered through the SLR
    \item Development of the search strings
    \item Selection of data sources 
    \item Definition of study selection criteria
\end{enumerate}

\subsubsection{Defining the research scope}

Defining the research scope is one of the crucial steps in planning the SLR \cite{papaioannou2016systematic}. It helps to formulate research questions, generate search strings, and establish the boundaries of the research \cite{del2018systematic}. Therefore, in order to determine the scope of this SLR, we adopted the PICOC (Population, Intervention, Comparison, Outcome, and Context) framework \cite{papaioannou2016systematic} as shown in Table \ref{tab: picoc}. Once the scope was defined, it was used to determine the approach to following SLR phases.

% \begin{table*}{}
%   \caption{SLR scope derived by following the PICOC framework \cite{papaioannou2016systematic} according to Del et al. \cite{del2018systematic}}
%   \label{tab: picoc}
%   \begin{tabular}{ 
%    >{\centering\arraybackslash}m{2cm} 
%    >{\raggedright\arraybackslash}m{5cm} 
%    >{\raggedright\arraybackslash}m{7cm}  }
%     \toprule
%     \textbf{Concept} & \textbf{Definition \cite{papaioannou2016systematic}} & \textbf{SLR application}\\
%     \midrule
%     Population & The existing problem that the SLR is dealing with. & Access control/privacy policy generation from natural language techniques to reduce the repetitive, time-consuming workload of the system administrator. \\
%     \noalign{\vskip 4.5pt}
    
%     Intervention & Existing tools and techniques proposed to address the problem & GUI-based tools and NLP-based frameworks for access control policy generation. \\
%     \noalign{\vskip 4.5pt}
    
%     Comparison(s) & Techniques to contrast the intervention & Contrast between the GUI tools and NLP frameworks. \\
%     \noalign{\vskip 4.5pt}
    
%     Outcome & A measure to assess the knowledge and limitations of the considered articles & Existing interventions will be assessed by the measures such as the flexibility, customizability, expressiveness, etc. of GUI tools as well as the efficiency, accuracy, etc. of NLP-based policy generation techniques.  \\
%     \noalign{\vskip 4.5pt}
    
%     Context & The particular settings or areas of the population & Access control policy generation while improving the reliability, flexibility, expressiveness, and efficiency of existing policy generation tools to help the system administrator. \\
    
%     \bottomrule
%   \end{tabular}
% \end{table*}

\begin{table*}{}
  \caption{SLR scope derived by following the PICOC framework \cite{papaioannou2016systematic} according to Del et al. \cite{del2018systematic}}
  \label{tab: picoc}
  \begin{tabular}{ 
   >{\centering\arraybackslash}m{2cm} 
   >{\raggedright\arraybackslash}m{12.5cm}  }
    \toprule
    \textbf{Concept} & \textbf{SLR application}\\
    \midrule
    Population & Access control/privacy policy generation from natural language techniques to reduce the repetitive, time-consuming workload of the system administrator. \\
    \noalign{\vskip 4.5pt}
    
    Intervention & GUI-based tools and NLP-based frameworks for access control policy generation. \\
    \noalign{\vskip 4.5pt}
    
    Comparison(s) & Contrast between the GUI tools and NLP frameworks. \\
    \noalign{\vskip 4.5pt}
    
    Outcome & Existing interventions will be assessed by the measures such as the flexibility, customizability, expressiveness, etc. of GUI tools as well as the efficiency, accuracy, etc. of NLP-based policy generation techniques.  \\
    \noalign{\vskip 4.5pt}
    
    Context & Access control policy generation while improving the reliability, flexibility, expressiveness, and efficiency of existing policy generation tools to help the system administrator. \\
    
    \bottomrule
  \end{tabular}
\end{table*}


\subsubsection{Formulation of research questions}

According to the scope we identified in Table \ref{tab: picoc}, the objective of this SLR is, to investigate the prior work related to the top-down policy generation tools and frameworks built in order to help the system administrators. To achieve the aforementioned goal, we developed the following research questions (RQs). 

% \textbf{RQ1}: What are the challenges that the system administrator is facing in the access control policy management of an organisation?

\textbf{RQ1}: \rqone
% \textbf{RQ2}: What tools or frameworks exist to support the system administrator to generate and understand access control policies?

\textbf{RQ2}: \rqtwo
%\textbf{RQ3}: What are the limitations of the existing access control policy generation tools?       

As the starting point, RQ1 focuses on investigating the existing tools and frameworks that suppose to help the system administrator to generate policies, by taking over the repetitive, laborious configuration process. Then in RQ2, we aim to ascertain the limitations and usability challenges of the existing tools, in order to develop a novel and effective tool to generate access control policies using NL. 

\subsubsection{Development of the search strings}
\label{subsubsec: searchstrings}

We identified a search string that is more likely to be used to extract the literature relevant to the area of interest. We used 2 techniques to decide which keywords to be included in each search string. 
\begin{enumerate}
    \item Extract keywords from the literature used for an initial assessment in the area of access control/privacy policy generation.
    \item Decide the keywords based on the terminology used for population in the defined scope (PICOC framework - Table \ref{tab: picoc}).
\end{enumerate}
Based on the above two techniques, we decided our main keywords are "administrator", "access control", "privacy policy", "natural language" and "generation". Even though we are mainly focusing on the access control domain, we considered "privacy policy" as one of the main keywords. Because, in our initial literature assessment, we found that the potentially relevant publications can also be found in the privacy policy domain. Apart from the above main keywords, we added several other keywords into the mix based on the initial assessment of the literature. Those keywords and the rationale behind choosing those words are as follows.
\begin{itemize}
    % \item \emph{behaviour} and \emph{challenges}: system administrator's behavioural factors and their challenges are the reasons for security misconfigurations as discussed in the Section \ref{sec:intro}.
    \item \emph{relation extraction}: when extracting Access Control Policy (ACP) components from NL texts, the relation between the words of the policy sentences can be considered \cite{slankas2014relation}. 
    \item \emph{natural language interfaces}: interfaces built to guide the non-technical user to develop access control policies in natural language with the help of GUI components such as text box, radio buttons, check box, and drop-down menus \cite{brodie2006empirical}
    
    % \item \emph{human factors}: since we are focusing on the tools developed based on the human factors of the users
\end{itemize}

To make sure that the relevant literature were not overlooked, we considered the variations of spellings such as behavior and behavior, when building the search strings. Further, we used the wild card notation ("*") to include the different forms of the same word in the search process. For example, instead of using "administrator" we used "admin*" to represent different forms of the word such as "administrators", "admin", "administration" and "admins". However, due to the fact that some important literature were missed when we only focus on the administrator, we decided not to add the term "admin*" to the final search string.

According to the aforementioned criteria, the developed search string is as follows. 

% \textbf{RQ1}: "admin*" AND "access control" AND ("challenges" OR "behaviour" OR "behavior") 
\texttt{("access control" OR "privacy policy" OR "privacy policies") AND ("natural language" OR "relation extraction" OR ("natural language" AND "generat*") OR ("natural language" AND "interfaces"))}

% We intentionally avoid using the term "admin*" in the second search string to extract all the publications related to policy generation from NL, even though it does not involve the administrator. 

\subsubsection{Selection of data sources}
\label{subsubsec: datasources}

Publications were extracted from two main sources, 1) Scientific digital libraries and 2) Top-tier selected cybersecurity conferences. 

As the scientific digital library we mainly considered  ACM Digital Library\footnote{https://dl.acm.org}, IEEE Xplore Digital Library\footnote{https://ieeexplore.ieee.org/Xplore/home.jsp}, Springer Link\footnote{https://link.springer.com}, and Elsevier Science Direct\footnote{https://www.sciencedirect.com}. Google Scholar\footnote{https://scholar.google.com} was used only to extract publications in Phase 3 of Section \ref{subsubsec: studySelect}. We found that the way we should define the search string for each search engine is different. For instance, ACM provides means to enter keywords in the search string separately and filter the literature based on the venue, even though Google Scholar only allows the user to enter the complete search string in the search box. Further, in the libraries such as IEEE Xplore and ACM, the user can decide where to search for a specific keyword in the research paper or article. For example, we can search literature by using keywords that appeared only in the abstracts, title, or anywhere in the document.   

To search for exact matches for the search string keywords, quotation marks ("") were used (e.g. "access control"). In addition, to ensure the keywords are searched together we combined the keywords with boolean operators such as AND. Even though we only used the AND and OR operators, the other basic operator (NOT) is also available in the above platforms to be used. 

Apart from the literature we extracted from the scientific digital libraries, we searched through the top-tier selected cybersecurity, human-computer interaction (HCI) as well as natural language processing conferences and journals, relevant to the topics in this SLR. Even though this SLR is not directly related to Human-Computer Interaction (HCI), we considered such conferences because the policy generation component involves natural language processing techniques to translate human intentions to machine (computer) executable policy. We selected 8 conferences and journals namely, IEEE Symposium on Security and Privacy (IEEE S\&P), USENIX Security, ACM Conference on Computer and Communications Security (CCS), ACM Transactions On Privacy and Security (ACM TOPS), Transaction of the Association for Computational Linguistics (TACL), Network and Distributed System Security Symposium (NDSS), ACM Conference on Human Factors in Computing Systems (CHI), Symposium on Usable Privacy and Security (SOUPS) and Conference on Empirical Methods in Natural Language Processing (EMNLP). The Breakdown of the selected venues is shown in Table \ref{tab: venues}. Search strings had to be changed by replacing AND with a "+" and OR with a " " (a space) while searching in USENIX\footnote{https://www.usenix.org/publications/proceedings}.

\begin{table*}[]
  \caption{Selected venues}
  \label{tab: venues}
  \begin{tabular}{ 
   >{\centering\arraybackslash}m{2cm} 
   >{\centering\arraybackslash}m{4cm} 
   >{\centering\arraybackslash}m{2cm}
   >{\centering\arraybackslash}m{2cm}}
    \toprule
    \textbf{Type} &  \textbf{Cybersecurity} & \textbf{HCI} & \textbf{NLP}  \\
    \midrule
    Conferences & IEEE S\&P, CCS, NDSS, SOUPS & CHI & EMNLP\\
         \noalign{\vskip 4.5pt}
         Journals & USENIX, ACM TOPS & - & TACL\\
    
    \bottomrule
  \end{tabular}
\end{table*}

\subsubsection{Definition of study selection criteria}
The study selection criteria help to determine what studies should be included and excluded from the SLR \cite{kitchenham2004procedures, fink2019conducting}. Therefore we defined the inclusion (IN) and exclusion (EX) criteria as shown in Table \ref{tab: criteria} to be relevant according to the scope in Table \ref{tab: picoc}.

% \textbf{IN1}: The publication which explains the challenges of the system administrator and their behavioural factors that affect to the policy configuration process.


\begin{table*}[]
  \caption{Inclusion and Exclusion Criteria}
  \label{tab: criteria}
  \begin{tabular}{ 
   >{\centering\arraybackslash}m{1cm} 
   >{\raggedright\arraybackslash}m{13cm}}
    \toprule
    \textbf{ID} &  \textbf{Criteria}\\
    \midrule
    IN1 & The publication presents the access control/privacy policy generation method from natural language policies or a method to guide users to generate and understand access control or privacy policies.\\

         IN2 & The publication presents a top-down policy engineering framework.\\

         IN3 & The publication should be related to access control or privacy/security policy configuration\\

         IN4 & The publication has been peer-reviewed.\\ 

         IN5 & The publication was written in English.\\
         \noalign{\vskip 4.5pt}
         \midrule
         \noalign{\vskip 4.5pt}
         EX1 & The publication is a secondary study.\\

         EX2 & The publication only presents a NLP technique for information extraction without applying it to access control or privacy policy domain.\\

         EX3 & The publication mainly focuses on an access control model, but not on a policy authoring guidance or an automation solution.\\

         EX4 & The publication focuses on social network privacy/access control policy configuration.\\

         EX5 & The publication presents a bottom-up policy mining/text mining approach.\\

         EX6 & The publication focuses on information extraction from privacy notices.\\
    
    \bottomrule
  \end{tabular}
\end{table*}


% \textbf{IN1}: The publication presents the access control/privacy policy generation or information extraction method from natural language policies or a method to guide users to generate and understand access control or privacy policies

% % access control policy visualisation techniques

% \textbf{IN2}: The publication presents a top-down policy engineering framework

% \textbf{IN3}: The publication has been peer-reviewed

% % \textbf{IN4}: The publication contains a working prototype which was evaluated using either well-recognized metrics or/and a user study

% \textbf{IN4}: The publication was written in English

% \textbf{IN5}: The publication propose a solution that can be employed by system administrators

% \textbf{EX1}: The publication is a secondary study

% \textbf{EX2}: The publication only presents a NLP technique for information extraction without applying it to access control or privacy policy domain

% \textbf{EX3}: The publication focuses on a novel access control model, but not on a policy authoring guidance or an automation solution

% \textbf{EX4}: The publication focuses on social network privacy/access control policy configuration

% \textbf{EX5}: The publication presents a bottom-up policy mining/text mining approach


% Since we are focusing on generating machine-executable access control policies from high-level natural language policies/requirements, our research belongs to the top-down policy engineering domain \cite{alohaly2019automated,alohaly2021hybrid}. On the other hand, in the bottom-up approach, information from the existing access control system (i.e. roles, attributes, users, actions, resources, etc.) will be used to generate the high-level policy \cite{alohaly2021hybrid}. Therefore we excluded the publications that propose a bottom-up policy engineering/mining approach.

% It is worth noting that some search strings retrieved more than 5000 publications (mostly from Google Scholar). In such cases we sorted the publications according to the relevance and extracted the publications on the first 10 pages based on the above criteria for this study. 

\subsection{Conducting the review}
\label{subsec:conductingSLR}

\begin{figure*}[]
    \centering
    \includegraphics[height=10cm]{images/PRISMA.png}
    \caption{PRISMA Flow diagram summarizing the research identification and study selection process}
    \label{fig:prisma}
\end{figure*}

After planning, SLR is conducted. As suggested by \cite{kitchenham2004procedures}, we performed 3 main activities called \emph{research identification and extraction, data synthesis, and data analysis}. 

\subsubsection{Research identification and Study Selection}
\label{subsubsec: studySelect}

This activity was performed during November - December 2022 under 3 main phases according to the PRISMA framework \cite{page2021prisma} as shown in Fig. \ref{fig:prisma}. 
\begin{itemize}
    \item \textbf{Phase 1: Digital Library Search - }We searched each library mentioned in the Section \ref{subsubsec: datasources} by applying the search strings developed under the Section \ref{subsubsec: searchstrings}.

    \item \textbf{Phase 2: Conference and Journal Search - }In order to avoid the publication bias \cite{kitchenham2004procedures}, we scanned through the selected journals and conferences mentioned in Section \ref{subsubsec: datasources} by applying the search strings developed under the Section \ref{subsubsec: searchstrings}.

    \item \textbf{Phase 3: Backward Snowballing Search - }To ensure the relevant publications are not overlooked, we searched through the references and citations in the retrieved publication from Phase 1 and Phase 2. This method was suggested in \cite{wohlin2014guidelines}. 
\end{itemize}

In Phase 1 (Search across the Digital Libraries), the developed search string returned a total of 2355 publications from 2013 to 2023. Even though we limit our search from 2013 to 2023, it does not mean that we did not consider relevant publications before 2013. Phase 3 allowed us to retrieve such publications using the backward snowballing technique. After removing duplicates using Zotero Reference Management Software\footnote{https://www.zotero.org}, a dataset of 1290 publications was obtained. Then 1290 extracted publications were further reviewed by reading the abstract, introduction, and sometimes the entire publication to decide whether to include it in the SLR or not. After removing the publications that do not match with inclusion and exclusion criteria, 23 publications were left as a result of Phase 1. 

Searching through the selected conferences and journals mentioned in Table \ref{tab: venues} was done under Phase 2. Our search was limited to publications from 2013. By using the same search strings, we extracted 23 potentially relevant publications. It is worth mentioning that, we were careful not to extract publications that were already extracted in Phase 1. Once the publications were reviewed, we obtained 10 publications after applying the inclusion criteria. 

Additional papers were identified by Backward Snowballing Search \cite{wohlin2014guidelines} in Phase 3. This method allows us to go through the references and citations mentioned in the publications obtained in Phase 1 and Phase 2. We extracted 20 relevant papers in this phase without any time limitations. At the end of Phase 3, we have a total of 53 publications retrieved by SLR. The summary of the research identification and study selection process is depicted in Fig. \ref{fig:prisma}, as suggested by \, cite{desolda2021human}.

\subsubsection{Data Extraction}

% The 53 publications which were obtained using the 3 phases mentioned in Section \ref{subsubsec: studySelect}, are listed in Table \ref{tab:pubs} sorted according to the surname of the first author. 

There are several observations were made while selecting and extracting the publications. Removing the search term "admin*" from the search string significantly increased the number of publications returned. Therefore we were able to extract publications that can potentially be helpful for the access control policy generation, even though they do not directly address the system administrator. Further, as we included the terms "privacy policies" and "privacy policy" into the search string, multiple publications which extract information from "privacy notices" such as data practices were returned. Since the returned publications were not related to the access control policy configuration domain, we decided to exclude them. However, privacy notices also contain natural language access control policies, that can be used to extract information for policy generation. Therefore, after careful consideration, we retained several publications related to the "privacy policy" domain that are focusing on extracting access control policies and/or their components. 
% Also, we observed that the techniques used in privacy policy domain show more advancement over the techniques used for access control policy generation. 
% \textcolor{blue}{Finally, it is worth mentioning that the most of the publications belong to the access control domain, do not contain the entire process from the NL access control policy to the machine executable policy. They basically pave the way towards the NL based policy generation by proposing methods to extract policy components.}

% \begin{table}[]
%     \centering
%     \begin{tabular}{p{2.5cm} p{1cm} p{2.5cm} p{1cm}}
%         \hlineB{2}
%         \noalign{\vskip 1.5pt}
%         {\textbf{Authors}} &  {\textbf{Reference}} & {\textbf{Authors}} & {\textbf{Reference}}  \\
%         \noalign{\vskip 1.5pt} 
%          \hline
%          \noalign{\vskip 3.5pt} 
%             Alohaly et al. & \cite{alohaly2018deep} & Reeder et al. & \cite{reeder2007usability}\\
% Alohaly et al. & \cite{alohaly2019automated} & Reeder et al. & \cite{reeder2008expandable}\\
% Alohaly et al. & \cite{alohaly2019towards} & Reeder et al. & \cite{reeder2011more}\\
% Alohaly et al. & \cite{alohaly2021hybrid} & Rosa et al. & \cite{rosa2020parser}\\
% Amato et al. & \cite{amato2013semantic} & Shen et al. & \cite{shen2021using}\\
% Basile et al. & \cite{basile2010ontology} & Shi et al. & \cite{shi2011controlled}\\
% Bertard et al. & \cite{bertard2020using} & Singru et al. & \cite{singru2020efficient}\\
% Brodie et al. & \cite{brodie2005usable} & Slankas et al. & \cite{slankas2012classifying}\\
% Brodie et al. & \cite{brodie2006empirical} & Slankas et al. & \cite{slankas2013access}\\
% Brostoff et al. & \cite{brostoff2005r} & Slankas et al. & \cite{slankas2013accessid}\\
% Cao et al. & \cite{cao2006intentional} & Slankas et al. & \cite{slankas2013implementing}\\
% Fatema et al. & \cite{fatema2016semi} & Slankas et al. & \cite{slankas2014relation}\\
% Fornara et al. & \cite{fornara2016modeling} & Stepien et al. & \cite{stepien2009non}\\
% Heaps et al. & \cite{heaps2021access} & Stepien et al. & \cite{stepien2014non}\\
% Inglesant et al. & \cite{inglesant2008expressions} & Tanoli et al. & \cite{tanoli2018towards}\\
% Johnson et al. & \cite{johnson2010optimizing} & Turner et al. & \cite{turner2017proposed}\\
% Johnson et al. & \cite{johnson2010usable} & Vanbrabant et al. & \cite{vanbrabant2009federated}\\
% Karat et al. & \cite{karat2006evaluating} & Vanbrabant et al. & \cite{vanbrabant2011fine}\\
% Maxion et al. & \cite{maxion2005improving} & Vaniea et al. & \cite{vaniea2008access}\\
% Morisset et al. & \cite{morisset2018building} & Vaniea et al. & \cite{vaniea2008evaluating}\\
% Morisset et al. & \cite{morisset2018visabac} & Xia et al. & \cite{xia2022automated}\\
% Narouei et al. & \cite{narouei2015automatic} & Xiao et al. & \cite{xiao2012automated}\\
% Narouei et al. & \cite{narouei2015towards} & Yang et al. & \cite{yang2021purext}\\
% Narouei et al. & \cite{narouei2017identification} & Ye et al. & \cite{ye2016identify}\\
% Narouei et al. & \cite{narouei2017towards} & Zhu et al. & \cite{zhu2021unstructured}\\
% Narouei et al. & \cite{narouei2018automatic} & Zurko et al. & \cite{zurko1999user}\\
% Perry et al. & \cite{perry2013modular} &  & \\
% \noalign{\vskip 3.5pt} 
%          \hlineB{2}
         
%     \end{tabular}
%     \caption{Obtained 53 publications selected for the SLR}
%     \label{tab:pubs}
% \end{table}

In order to extract necessary data, the first author examined each of the obtained publications. From each publication, the lead author collected general quantitative data (e.g. title, author, year, published venue, etc. ) as well as the qualitative information that aligns with the formulated research questions in Section \ref{subsec:planning}. 
% Even though, he reviewed the entire publication, he focused on several particular sections in the publication to extract necessary information to answer the research questions. 

% \begin{itemize}
%     \item \emph{RQ1}: Abstract, Introduction, Proposed methodology, Conclusion.
%     \item \emph{RQ2}: Threats to validity, Challenges, Experimental Results, Evaluation, Discussion, Related Works, Conclusion.
    
% \end{itemize}

\subsection{Data Analysis}
\label{subsubsec: data_analysis}

Since we aim to answer the research questions by identifying recurring patterns of meaning and concepts within the extracted data, next, we conducted \textbf{Thematic Analysis} \cite{cruzes2011recommended} according to the following steps. 

\begin{enumerate}
    \item \emph{Familiarisation}: Extracted data was read and summarised using the Mendeley Reference Management Software\footnote{https://www.mendeley.com} to have an overview of the data. Here we used Mendeley instead of Zotero, as it offers more advanced annotation and note-taking features than Zotero.
    \item \emph{Generating Codes}: As we are coding with specific research questions in mind, we followed the integrated coding procedure \cite{cruzes2011recommended}. The first author was in charge of assigning codes that reflect the relevant features to answer the research questions. 
    % However, we did not use line-by-line coding technique as the first author was supposed to code more than 50 publications. Instead of line-by-line coding he relied on extracted data and the written summary to assign codes. 
    For instance, the first author assigned the code \emph{"parsing"} to the text in the extracted information \emph{"In our approach, after identifying the different sentence types, we parse each line (sentence) using the Stanford  Natural Language Parser and output a graph in the  Stanford Type Dependency Representation (STDR)."} \cite{slankas2014relation}. Furthermore, the extracted data were read multiple times to refine the generated codes and to determine whether they were assigned correctly.
    \item \emph{Generating initial themes}: All the codes were compiled into logical groups to identify themes that help to answer the research questions. 
    \item \emph{Reviewing the themes}: Initial themes were checked against the data segments extracted and refined to create the final set of themes. 
    \item \emph{Defining and naming higher order themes}: The relationships between the initial themes were used to define overarching higher order themes with a meaningful name and a detailed description. 
    % For instance, the themes for RQ1 were generated based on the policy authoring guidance and automation solutions. (e.g. GUI based policy authoring, Natural language based policy translation)
\end{enumerate}

In the end, the co-author validated the process by reviewing the consistency of codes and themes against the associated data and examining whether the generated themes and categories respond to the research questions RQ1 and RQ2. Several meetings were conducted involving the three authors to discuss the disagreements and issues of generated codes and themes. As result, we minimized the possible inconsistencies in the coding process.

Once the themes and categories were generated, the main author filled out a spreadsheet to classify the articles based on the detailed descriptions of the themes/categories. Later, the agreements and disagreements of the other coders regarding the classification decisions were expressed and recorded in a meeting to calculate the metrics for inter-rater reliability (i.e. Cohen kappa ($\kappa$) \cite{viera2005understanding} and percentage of agreement). After the calculation, we noticed that the co-authors a "near perfect agreement" ($\kappa$ $\geq$ 0.81) and a percentage agreement above 80\% at classifying articles into the defined categories. However, we came across several disagreements on classifying based on the GUI-based configuration tools (authoring vs. visualization tools). We discussed the disagreements in a meeting and resolved them by examining the descriptions of the categories.     

% Upon following the above steps, we developed a \emph{Thematic Tree} containing the generated higher order themes and sub-themes as shown in the Fig. \ref{fig:tools}.

\section{Results}

% This section reports the analysis results of extracted publications according to the formulated research questions in Section \ref{subsec:planning}.

As a result of the thematic analysis \cite{cruzes2011recommended}, we identified 2 main approaches taken by previous literature to develop tools and frameworks that help the system administrator to generate and understand access control policies as shown in Fig. \ref{fig:tools}. They are graphical policy authoring and visualization \cite{stepien2014non, brostoff2005r, zurko1999user, vaniea2008access, johnson2010optimizing, maxion2005improving, cao2006intentional, reeder2007usability, reeder2008expandable, morisset2018visabac,stepien2009non, reeder2011more, morisset2018building, bertard2020using, rosa2020parser, turner2017proposed}, and NLP-based automated policy generation \cite{fatema2016semi,xiao2012automated,slankas2012classifying,ye2016identify,slankas2013implementing,fornara2016modeling,perry2013modular,slankas2014relation,jones2015towards,tanoli2018towards,amato2013semantic,slankas2013access,slankas2013accessid,rosa2020parser,brodie2006empirical,alohaly2016better,vaniea2008evaluating,karat2006evaluating,inglesant2008expressions,basile2010ontology,turner2017proposed,reeder2007usability,brodie2005usable, vanbrabant2011fine,das2018hype,shen2021using,xia2022automated}.

 Tools used for graphical policy authoring and visualization often provide a usable interface that allows system administrators to write and visualize policies manually. Previous literature proposed graphical user interfaces (GUIs) specifically designed for policy authoring, such as text editor-based \cite{brostoff2005r, zurko1999user, stepien2009non, stepien2014non} and template-based authoring tools \cite{johnson2010optimizing, johnson2010usable, rosa2020parser, turner2017proposed}, tools designed for policy visualization, such as graph-based visualization tools \cite{morisset2018building, morisset2018visabac, bertard2020using}, and tools that facilitate both policy authoring and visualization at the same time, such as access matrix-based policy authoring and visualization tools \cite{reeder2008expandable, reeder2011more, vaniea2008access, cao2006intentional, maxion2005improving, vaniea2008evaluating}. Text editor-based tools guide the administrator to build a policy by separately defining its policy components using text boxes \cite{stepien2009non, stepien2014non} or combo boxes \cite{brostoff2005r}. On the other hand, template-based tools provide one \cite{turner2017proposed, rosa2020parser} or more pre-defined templates \cite{johnson2010usable, johnson2010optimizing} to write the policy according to a common format while preserving the semantic meaning of the intended policy. However, neither of those types of tools visualizes the already written policies and their rules graphically. Therefore, the important contextual information, that is essential, especially when resolving conflicts between policies from all the policies will not be available to the administrator \cite{reeder2008expandable}. With that in mind, access matrix-based tools that allow the administrator to write as well as visualize all the policies in a single matrix (representing users as rows and resources as columns) were developed \cite{reeder2008expandable, reeder2007usability, maxion2005improving}.  However, the access matrices can be hard to navigate if the number of users and resources is high in the organization \cite{morisset2018building}. As a solution, graph-based visualization tools were proposed to effectively represent the high number of users and resources in the organization \cite{morisset2018visabac}. Overall, these tools provide a higher level of abstraction allowing administrators to focus on the high-level access control requirements of the organization rather than low-level technical details of the access control model, language, or syntax. 
 % Therefore, many studies have shown that these tools improve efficiency, and accuracy while reducing the cognitive load in policy configuration \cite{reeder2008expandable, reeder2011more, karat2006evaluating, maxion2005improving, stepien2009non, stepien2014non}. 
 However, the proposed graphical tools have their own limitations. As we found out, some of the graphical policy authoring tools lack the flexibility \cite{brodie2006empirical, brodie2005usable, karat2006evaluating, vaniea2008access, turner2017proposed, rosa2020parser, shi2011controlled, inglesant2008expressions} and do not support complex access control policies \cite{stepien2009non, stepien2014non, bertard2020using, morisset2018building, morisset2018visabac, reeder2008expandable, reeder2011more, maxion2005improving, cao2006intentional}, preventing the administrator to build custom and complex policies with different access requirements. Furthermore, the graphical representation of the policies as well as the GUI features of the tools often are subjected to inconsistent interpretations by the administrators depending on their expertise in access control \cite{brostoff2005r, morisset2018building, morisset2018visabac}. These limitations make the existing graphical policy authoring and visualization tools less effective in generating access control policies.

Nevertheless, graphical policy authoring and visualization is a manual, repetitive, and laborious process \cite{narouei2015automatic}. Therefore, IT security professionals consider this process as an overhead \cite{botta2007towards} which can cause fatigue and stress impairing their critical decision-making ability \cite{palmer_2021}. As a solution NLP-based automated policy generation frameworks were introduced, that utilize ML and NLP techniques to translate high-level policy documents into machine-executable policies without any human involvement. The proposed frameworks consist of 5 main steps. First, the NL document were pre-processed by using techniques such as sentence tokenization \cite{slankas2012classifying, slankas2013access, slankas2013accessid, slankas2014relation, narouei2015automatic, narouei2015towards, narouei2017identification, narouei2017towards, narouei2018automatic, tanoli2018towards, xiao2012automated}, word tokenization \cite{narouei2015automatic, narouei2015towards, narouei2017identification, narouei2017towards, narouei2018automatic, alohaly2018deep, alohaly2019automated, alohaly2019towards, tanoli2018towards, heaps2021access, yang2021purext, singru2020efficient, amato2013semantic}, filtering unwanted sections in the document \cite{slankas2012classifying, slankas2013access, narouei2017identification, narouei2017towards}, stop word removal \cite{tanoli2018towards, singru2020efficient} etc. Secondly, the natural language access control policies were identified using text classification techniques such as Support Vector Machines (SVM) \cite{slankas2013access, slankas2013accessid}, k-Nearest Neighbours \cite{slankas2014relation, slankas2012classifying, slankas2013access, slankas2013accessid, narouei2015automatic, narouei2018automatic, narouei2015towards}, Transformers \cite{heaps2021access, xia2022automated}, Naive Bayes \cite{slankas2013access, narouei2017identification} etc. Once the NLACPs were identified, machine-executable policies should be built from the NLACPs. Therefore, as the third step, necessary policy components (i.e. subjects, actions, resources, etc.) were extracted by employing information extraction techniques including syntactic parsing \cite{brodie2006empirical, xiao2012automated, vaniea2008evaluating, karat2006evaluating, reeder2007usability, brodie2005usable, slankas2013access, narouei2017identification, ye2016identify, yang2021purext, slankas2014relation, alohaly2019towards, tanoli2018towards, xia2022automated, shi2011controlled, fatema2016semi, inglesant2008expressions, vanbrabant2009federated, vanbrabant2011fine, turner2017proposed, shen2021using, basile2010ontology, alohaly2018deep, alohaly2019automated}, semantic role labeling (SRL) \cite{xia2022automated, narouei2015automatic, narouei2018automatic, yang2021purext, narouei2017towards, narouei2015towards}, named entity recognition (NER) \cite{heaps2021access, zhu2021unstructured} or a combination of multiple extraction techniques (e.g. SRL and dependency parsing were used together to extract component in a more granular way \cite{xia2022automated, narouei2015automatic, yang2021purext, narouei2015towards, alohaly2019towards}). As the fourth step, the extracted policy components were transformed into a policy language such as XACML (eXtensible Access Control Markup Language) \cite{xia2022automated, turner2017proposed, amato2013semantic, slankas2012classifying, fatema2016semi, vanbrabant2011fine, brodie2005usable, vaniea2008evaluating, shi2011controlled, karat2006evaluating, brodie2006empirical}, PERMIS (Policy Enforcement through Role-based access control Mechanisms Implementation and Specification) \cite{inglesant2008expressions, shi2011controlled}, EPAL (Enterprise Privacy Authorization Language) \cite{brodie2006empirical, brodie2005usable, karat2006evaluating, vaniea2008evaluating} or into an intermediate representation such as an ontology \cite{shi2011controlled, inglesant2008expressions, fornara2016modeling, tanoli2018towards, basile2010ontology}. Finally, the generated policies were evaluated either by using the F1-score \cite{xiao2012automated, xia2022automated, slankas2013access, slankas2013accessid, slankas2012classifying, slankas2014relation, narouei2015towards, narouei2017towards, narouei2018automatic, narouei2017identification, alohaly2018deep, alohaly2019automated, alohaly2019towards, heaps2021access, brodie2006empirical, shen2021using, yang2021purext, zhu2021unstructured} or the accuracy \cite{singru2020efficient} in the extracted literature. Since human involvement is minimum in the above five steps, the room for human errors is minimum. Furthermore, the policy generation process will be more efficient than the manual policy generation, since the entire process is done by an algorithm.

Despite helping the administrator by automating the policy generation, we identified several limitations of existing policy generation frameworks. Our study revealed that the lack of domain-related high-quality datasets hinders the development of more accurate frameworks \cite{nobi2022machine, xia2022automated}. Also, it makes the existing automated policy generation frameworks not reliable or granular enough to operate without human supervision \cite{del2022systematic, xia2022automated, narouei2015automatic}. Furthermore, some of the existing frameworks, especially the ones that use rule-based information extraction techniques \cite{xiao2012automated, brodie2006empirical} cannot handle ambiguities in NLACPs making the rule-based parsers fail to identify policy components in sentences that are ambiguous. Therefore, to avoid ambiguities previous literature decided to use a controlled natural language (CNL) that forces administrators to write policies according to pre-defined syntax or templates, restricting the allowed vocabulary and grammar \cite{brodie2006empirical, inglesant2008expressions, shi2011controlled}. However, this restriction limits the flexibility of policy authoring, making it difficult for administrators to transfer their intended policies to the authorization system \cite{inglesant2008expressions}. 

According to the above overview of our results, even though graphical policy authoring and visualization tools guide the administrator to write policies correctly, their own limitations make them less usable for effective policy authoring and visualization. Furthermore, the manual and repetitive graphical policy authoring techniques significantly contribute to the overhead of administrators due to the lack of automation. On the other hand, even though the NLP-based automated policy generation frameworks reduce that overhead significantly, they cannot be used without human supervision (i.e. lack of human involvement). Therefore, to develop a more effective tool, it is important to identify how the existing graphical policy authoring and visualization tools and NLP-based automated policy generation frameworks can be further improved and how to combine them in a way that they complement each other. With that in mind, in the next two subsections, we discuss graphical policy authoring and visualization tools, and NLP-based automated policy generation frameworks as the answer to our first research question RQ1, and their limitations as the answer to our second research question RQ2.


\subsection{\rqone\ (RQ1)}
\label{subsec: tools_frameworks}

As we briefly mentioned above, we identified 2 types of tools and frameworks that were developed to help the system administrator in generating access control policies.

\begin{enumerate}
    \item Graphical policy authoring and visualization tools.
    \item NLP-based automated policy generation frameworks.
\end{enumerate}

Therefore, under this section, we first discuss the unique features of graphical policy authoring and visualization tools \cite{stepien2014non, brostoff2005r, zurko1999user, karat2006evaluating, johnson2010usable, johnson2010optimizing, maxion2005improving, cao2006intentional, reeder2007usability, reeder2008expandable, morisset2018visabac, shi2011controlled,stepien2009non, reeder2011more, morisset2018building, besmer2010impact, bertard2020using, inglesant2008expressions, rosa2020parser, turner2017proposed, brodie2005usable, brodie2006empirical, vaniea2008evaluating}. 
% in terms of text editor-based policy authoring, template-based policy authoring, access matrix-based policy authoring and visualization, and graph-based policy visualization tools.
Secondly, we explain the techniques used to build the NLP-based automated policy generation frameworks \cite{fatema2016semi,xiao2012automated,slankas2012classifying,ye2016identify,slankas2013implementing,fornara2016modeling,perry2013modular,slankas2014relation,jones2015towards,tanoli2018towards,amato2013semantic,slankas2013access,slankas2013accessid,rosa2020parser,brodie2006empirical,alohaly2016better,vaniea2008evaluating,karat2006evaluating,inglesant2008expressions,basile2010ontology,turner2017proposed,reeder2007usability,brodie2005usable, vanbrabant2011fine,das2018hype,shen2021using,xia2022automated}. 
% which consist of 5 main steps: pre-processing, text classification, information extraction, information transformation, and evaluation. 

\begin{figure*}[]
    \centering
    \includegraphics[height=17.5cm]
    {images/themes.png}
    
    \caption{Thematic map showing the identified access control policy generation approaches. Under RQ1, we discuss GUI-based policy generation in terms of policy authoring and visualization tools, and NLP-based policy generation frameworks in terms of preprocessing techniques, text classification techniques, information extraction techniques, information transformation techniques, and evaluation techniques. Under RQ2, we discuss the limitations of identified GUI-based tools and NLP techniques.}
    \label{fig:tools}
\end{figure*}

% Thematic map of the themes discussed in the SLR categorized according to the research questions RQ1 and RQ2

\subsubsection{Graphical policy authoring and visualization}
\label{subsubsec: gui}

\begin{figure*}[]
    \centering
    \includegraphics[height=9cm]{images/guis.png}
    \caption{Examples for GUI-based policy authoring and visualization tools: (a) "easyXACML" text-editor-based tool \cite{stepien2009non}, (b) "Expandable Grids" access matrix-based visualization tool \cite{reeder2008expandable, reeder2011more}, (c) "Salmon": access-matrix-based tool \cite{maxion2005improving}, (d) Template-based tool by Johnson \cite{johnson2010usable}, (e) "VisABAC" visualization tool \cite{morisset2018building}}
    \label{fig:gui_tools}
\end{figure*}

% Complexity of the policy configuration system together with the repetitive, tedious nature of the configuration process 

% Authoring policies directly in a machine-executable language such as XACML (eXtensible Access Control Markup Language), is prone to mistakes resulting in access control configuration failures \cite{stepien2014non, lorch2003first}. For example, when writing a policy in XACML, the system administrator has to follow a strict syntax structure containing multiple nested XML tags such as \texttt{<Policy> <Target> <AnyOf> <AllOf> </AllOf> </AnyOf> </Target> </Policy>}. If the administrator did not follow that proper tag structure and more importantly the administrator is not fluent in XACML, it will result in an incorrect access control policy which may cause access control failures \cite{stepien2009non}. 

% Furthermore, those policy languages do not often provide means to visualize the written access control policies and rules, so that the administrator can identify the relationships and conflicts between them \cite{lorch2003first}. Consequently, resolving conflicts between policies will be difficult.

% Therefore, to guide the administrator to write and visualize access control policies without worrying about the underlying policy languages, syntax, or models, graphical policy authoring and visualization techniques were developed \cite{stepien2009non, reeder2008expandable, johnson2010usable, morisset2018visabac}. 

According to our thematic analysis \cite{cruzes2011recommended}, 45.1\% of the included publications proposed graphical user interfaces (GUIs) to guide administrators in access control policy configuration. On the one hand, several publications proposed text editors \cite{stepien2009non, stepien2014non, brostoff2005r, zurko1999user, shi2011controlled, inglesant2008expressions} and template-based authoring tools \cite{johnson2010optimizing, johnson2010usable, rosa2020parser, turner2017proposed, brodie2005usable, brodie2006empirical, karat2006evaluating, vaniea2008evaluating} to guide administrators to write access control policies without even having knowledge about policy languages such as XACML. On the other hand, some developed graphs \cite{morisset2018building, morisset2018visabac, bertard2020using} and access matrices-based \cite{reeder2007usability, reeder2008expandable, maxion2005improving, cao2006intentional, vaniea2008access} policy visualization tools that allow the administrator to visualize the policies. Therefore under this theme, we discuss the above types of graphical policy authoring and visualization tools and their unique features as we identified in the SLR.

\textbf{Text editor-based policy authoring} - Among the identified graphical policy authoring and visualization tools, 22.7\% of them are text editor-based policy authoring tools. Instead of forcing the administrator to write the access control policy directly in a policy language, policy editors provide means of building the policy just by inputting the values for respective policy components (i.e. subject, actions, resource, etc.) in separate text boxes \cite{brostoff2005r, zurko1999user, stepien2009non, stepien2014non}. The policy component inputting can either be done by entering each policy component value in the text boxes \cite{stepien2009non, stepien2014non, zurko1999user} or by choosing the provided values from a drop-down menu or combo box \cite{brostoff2005r}. For instance, the interface developed by Stepien et al. \cite{stepien2009non, stepien2014non} provides text boxes for each policy component, to type the respective values as shown in Fig. \ref{fig:gui_tools}(a) while Brostoff et al. allow the administrator to choose already existing values extracted from LDAP directory structure \cite{brostoff2005r}. Therefore, if administrators can identify what the subjects, actions, resources, and conditions of the policy are, they can add those values in the correct text boxes to generate the machine-executable policy.

% However, system administrators sometimes lack the understanding of what the relevant policy components are in their intended policies (i.e. what subjects, actions and resources are relevant to build the policy) \cite{brostoff2005r}. Therefore it would be easier, if the interface guide them to translate their access control policy in mind, to a predefined structure. For example, the policy \emph{"The fileA can be written by the CEO and the manager but not employees"} has one resource (i.e. fileA), one action (i.e. write), and three subjects (i.e. CEO, manager, and employees). Therefore, the administrator has to correctly identify two access control rules that allow the manager and the CEO to write fileA and one other rule that restricts employees from writing to the fileA. If the administrator fails to identify these components and rules to enter in the respective text boxes, it will cause access control failures leading to drastic data breaches \cite{Holmes_2021}. Furthermore, the administrator has to manually repeat the process 3 times to write the above policy. Therefore, as a solution, template-based policy authoring interfaces were introduced that allow the administrator to write the entire policy at once in a text box according to a predefined structure, without breaking it down into single policy components.


\textbf{Templates-based authoring} - Properly formatted high-quality access control policies often increase the manageability of the policy configuration system \cite{bertino2018challenge}. For example, when there are multiple policy authors involved in policy configuration, having policies with consistent format helps to avoid confusion between the policies written by multiple authors \cite{bauer2009real}. Therefore, in order to guide the policy authors (i.e. system administrator) to write properly formatted policies according to pre-defined policy structures, template-based policy authoring interfaces were introduced \cite{johnson2010optimizing, johnson2010usable, rosa2020parser, turner2017proposed, brodie2005usable, brodie2006empirical, karat2006evaluating, vaniea2008evaluating}. 
% Templates not only help the administrators to express their intentions clearly but also they act as a guide to inexperienced administrators. 

A template is a specification of the structure of a list of natural language policies \cite{johnson2010usable}. Once the templates are defined, administrators can choose policy components for the placeholders of the template so that the completed policy is semantically matched with their intended access control policy. For example, to write a policy, \emph{"It is prohibited that a contractor or volunteer in the cardiology department to view medical records that belong to heart patient"}, Turner provided a template \texttt{It is \{Decision\} that a(n) \{Subject\} who is in the \{Department\} \{Action\} a(n) \{Target\} that belongs to a(n) \{Owner\}} in his template-based authoring interface, "XpressRules" \cite{turner2017proposed}. However, a single template would not be enough to support all the policy requirements of an organization. Therefore, in their template-based policy authoring interface shown in Fig. \ref{fig:gui_tools}(c) Johnson et al. have allowed to create and modify new templates depending on the requirements of the organization \cite{johnson2010optimizing, johnson2010usable}. As a result, they were able to improve the flexibility of the template-based policy authoring interface by supporting an unlimited number of policy structures.


\textbf{Access Matrix-based policy authoring and visualization} - "Access control matrix" is the most common type of interface we identified that not only guides the administrator to configure access control policies but also visualizes them in a matrix. It was first introduced by Lampson \cite{lampson1974protection}. Lampson's access control matrix was originally represented as a two-dimensional table, where each row represents a subject, each column represents a resource, and each cell contains the set of operations that the subject is allowed to perform on the object. Thereafter, the access control matrix was used in several research with some improvements as a method of configuring and visualizing access control policies \cite{reeder2008expandable, reeder2011more, vaniea2008access, cao2006intentional, maxion2005improving, vaniea2008evaluating}. 
 % Interestingly, most of the extracted articles that propose access matrix-based authoring and visualization techniques attempted to solve limitations in Windows XPFP (XP File Permission) interface \cite{maxion2005improving, cao2006intentional, reeder2008expandable, reeder2011more}. For example, the XPFP interface follows the list-of-rules model, which displays the rules of a policy. However, it only allows the system administrator to select a single rule at a time for viewing or editing \cite{reeder2008expandable}. Since a policy could contain multiple rules, viewing or editing a single rule in isolation will make the important contextual information from the remainder of the policy unavailable to the administrator \cite{reeder2007usability}. As a result, it is difficult to identify the rules that conflict with each other since the other rules as not visible at the same time \cite{reeder2008expandable}. Therefore, as solutions, Maxion et al. introduced "Salmon" interface (Fig. \ref{fig:gui_tools}(c) \cite{maxion2005improving} and Cao introduced an interface for Intentional Access Management (IAM) \cite{cao2006intentional} based on the access matrix. In their access control matrix-based interfaces, all the rules contained in a policy for a given user/group are displayed in a matrix. The rows of the matrix were used to encode users and groups of the organization, while the columns were used to denote atomic permissions such as executing a file, reading data, writing attributes, etc. for the selected resource (i.e. a file/folder). Therefore, if the administrator wants to provide "execute file" permission to a user, the administrator just need to choose the file, select the user from the access matrix and tick the box at the intersection of the user row and "execute file" column. Furthermore, not only the stated permission (i.e. permission for an individual user) the "Salmon" interface also displays effective permission (i.e. permission derived from the user's individual permission and the permission of groups that the user belongs to) for the selected user in the bottom part of the interface as shown in Fig. \ref{fig:gui_tools}(c). Since all the rules of policies and their relationships can be seen and edited in a single interface with all the information, Maxion and Cao were able to solve the limitations of list-of-rule model used by the XPFP interface \cite{cao2006intentional, maxion2005improving}. 
For example, Reeder et al. proposed "Expandable Grids" (Fig. \ref{fig:gui_tools}(b)) \cite{reeder2008expandable, reeder2011more} by following the original Lampson's access matrix \cite{lampson1974protection}. They encoded all the principals and their associated groups in rows and all the resources and associated resource groups in the system were assigned to the columns. In contrast to the other access matrix-based interfaces, Expandable Grids uses a sub-grid in each cell to authorize each user to read, write, delete, execute, and administrate resources. To represent whether the above 5 actions are allowed, denied, or some access allowed when a user inherits access from a group (i.e. effective permission), green, red, and yellow colors were used respectively as shown in Fig. \ref{fig:gui_tools}(b).

Even though the access matrix-based visualization works well for a fairly small amount of users and resources, the navigation through the axes (users and resources) will become quite tedious when there are many users and resources exist in the system \cite{morisset2018visabac, morisset2018building}. As a solution, graph-based visualization techniques were proposed.

\textbf{Graph-based policy visualization} - Graphs/trees can be in different forms such as layered graphs, hierarchical graphs, hypergraphs, Euler diagrams, binary decision diagrams, and treemaps. By considering the aforementioned alternatives, graph/tree-based techniques were also proposed in previous literature to visualize access control policies \cite{morisset2018building, morisset2018visabac, bertard2020using}. Morisset et al. introduced a treemap-based visualization tool, "VisABAC" to visualize the interaction among rules and policies in an ABAC policy \cite{morisset2018building, morisset2018visabac} as shown in Fig. \ref{fig:gui_tools}(e). They utilized a special form of treemaps named "Circular Treemap", which represents tree nodes as circles. For instance, a parent node with 2 children nodes will be represented as a circle containing 2 sub-circles in the circular treemap method. In the access control domain, the parent circle would be a policy, and the children circles would be policies or rules. As an additional usability feature, they made the circles zoomable, so that the administrator can zoom in and zoom out to get a better view of the polcy and its underlying rules \cite{morisset2018visabac, morisset2018building}. Moreover, to visualize RBAC policies, Bertard et al. proposed a layered graph-based approach named "Sugiyama-styled Graph" in \cite{bertard2020using}. The proposed approach contains a graph with 3 layers representing the users, roles, and resources in the organization. Each layer has nodes per user, each role, and each resource respectively. 

The above graphical policy authoring and visualization techniques guide the administrator to write access control policies even without extensive knowledge on access control models, languages, or syntax \cite{stepien2009non}. However, the policy generation using those tools is a manual, repetitive, and laborious task, which is considered as an overhead by the security experts \cite{botta2007towards}. This overhead can lead to fatigue and stress in the system administrator increasing the likelihood of mistakes when configuring policies manually. For example, if administrators are tired and stressed after configuring policies repetitively, there is a chance that they might provide unauthorized access to a user by clicking the incorrect cell in an access matrix-based interface. As a solution, previous literature then proposed to remove the human factor entirely from the policy generation by proposing natural language processing (NLP) based automated policy generation frameworks \cite{fatema2016semi,xiao2012automated,slankas2012classifying,ye2016identify,slankas2013implementing,fornara2016modeling,perry2013modular,slankas2014relation,jones2015towards,tanoli2018towards,amato2013semantic,slankas2013access,slankas2013accessid,rosa2020parser,brodie2006empirical,alohaly2016better,vaniea2008evaluating,karat2006evaluating,inglesant2008expressions,basile2010ontology,turner2017proposed,reeder2007usability,brodie2005usable, vanbrabant2011fine,das2018hype,shen2021using,xia2022automated}. 


\subsubsection{NLP-based automated policy generation}
\label{subsubsec: nlpgen}

The main objective of the NLP-based automated policy generation process is to translate the Natural language access control policies (NLACPs) into low-level machine executable policies without human involvement. 
% We call this translation process as "top-down policy engineering". 
The process starts with the administrator's input. The input can either be a single NL access control policy (NLACP) or a requirement document containing multiple NL sentences. In the later input scenario, the document can contain both ACPs and non-ACPs. Therefore, in order to achieve a successful translation, 4 steps were followed in the analyzed publications. First, the input NL sentence(s) were pre-processed to make them ready for translation. Then the pre-processed sentence(s) were classified as NLACP or non-NLACP. Only the sentences identified as NLACPs were used for the translation. Once the NLACPs were identified, the policy components of the NLACP (e.g. subject, action, resource, purpose, etc.) or attributes (e.g. subject attributes, object attributes, environment attributes, etc.) were extracted. Finally, the extracted policy components or attributes were arranged as a machine-executable code. 

Under this subsection, we first report the common ML/NLP techniques used to facilitate the aforementioned steps identified as a result of the thematic analysis (See Fig. \ref{fig:tools}). Secondly, we report the publicly available datasets we found that can be used to train and evaluate future automated policy generation models.

\textbf{Pre-processing} - Pre-processing refers to the set of techniques that are used to clean, transform and prepare textual data before they can be used for further processing. Even though the pre-processing techniques are essential for ML/NLP tasks, only 39.2\% of the extracted publications explicitly mentioned the pre-processing techniques they used in the policy generation process, utilizing libraries such as CoreNLP tool kit \cite{manning2014stanford}, NLTK \cite{bird2006nltk}, and SpaCy\footnote{https://spacy.io/}.
% The pre-processing techniques and the previous literature that employed those techniques are as follows.

\begin{itemize}
    \item \emph{Sentence Tokenization}: The process of splitting the ACP sentences using punctuation marks indicating the sentence boundaries \cite{slankas2012classifying, slankas2013access, slankas2013accessid, slankas2014relation, narouei2015automatic, narouei2015towards, narouei2017identification, narouei2017towards, narouei2018automatic, tanoli2018towards, xiao2012automated}. This pre-processing step is necessary when processing documents containing NLACPs.

    \item \emph{Word Tokenization}: The process of breaking down a sentence into word tokens. Word tokenization, based on the white spaces is the most common technique used in the extracted literature \cite{narouei2015automatic, narouei2015towards, narouei2017identification, narouei2017towards, narouei2018automatic, alohaly2018deep, alohaly2019automated, alohaly2019towards, tanoli2018towards, heaps2021access, yang2021purext, singru2020efficient, amato2013semantic}. However, when it comes to languages other than English (e.g. Chinese), rule-based tokenization was employed \cite{shen2021using}. 

    \item \emph{Filtering}: The process of filtering the unwanted sections of NL requirement documents for NLACP extraction (i.e. titles, list items, headers, footers, etc) \cite{slankas2012classifying, slankas2013access, narouei2017identification, narouei2017towards}.

    \item \emph{Stemming and Lemmatization}: The process of reducing the words to their base form (e.g. liked, likes $\rightarrow$ like, caring $\rightarrow$ care) \cite{singru2020efficient, tanoli2018towards, amato2013semantic}.

    \item \emph{Parsing and Tagging}: In some cases, the NL sentence was parsed and tagged according to its grammatical structure before further processing. Parsing and tagging as a pre-processing technique was performed in terms of Part-of-Speech (POS) tagging \cite{amato2013semantic}, shallow parsing \cite{xiao2012automated}, dependency parsing \cite{slankas2012classifying, slankas2013access, slankas2013accessid, slankas2013implementing, slankas2014relation, amato2013semantic, narouei2017identification} and rule-based parsing \cite{perry2013modular}. 
    % However, most of the time parsing was used as an information extraction technique, which we discuss in a later topic. 

    \item \emph{Stop word removal}: The process of removing the most common words that do not carry a significant meaning such as "a", "an", "the" etc. \cite{tanoli2018towards, singru2020efficient}.

    % \item \emph{Embedding}: Embedding is a technique of encoding phrases of a sentence into numerical dense vectors. These vectors capture the semantic meaning of the underlying phrases so that the vectors of the phrases with similar meanings will be closer together in the vector space. Often the embeddings are used on the tokens before feeding them into a NLP model to associate the tokens with a semantic meaning. In the identified literature, researchers used several different embedding techniques pre-trained on different corpora such as GoogleNews, Common Crawl, Wikipedia, etc. to encode the words of NLACPs. For instance, Alohaly et al. \cite{alohaly2019automated, alohaly2018deep, alohaly2019towards} used GloVe word embeddings \cite{pennington2014glove}, Narouei et al. \cite{narouei2017towards} and Zhu et al. \cite{zhu2021unstructured} used Word2Vec embeddings \cite{mikolov2013efficient}, also the BERT (Bi-directional Encoder Representation for Transformers) \cite{devlin2018bert} embeddings were used by Heaps et al. \cite{heaps2021access} and Xia et al. \cite{xia2022automated}.   
\end{itemize}

Once the data were cleaned and properly formatted according to the discussed techniques, text classification techniques were applied to the resultant sentences to identify the ACP sentences.

\textbf{Text Classification} - Text classification is a NLP technique that assigns labels to textual segments based on certain criteria. In the access control policy generation process, text classification was mainly used to identify NLACPs in high-level access control requirement documents, as those documents might contain non-access control policies \cite{xiao2012automated, slankas2012classifying, slankas2014relation, slankas2013access, slankas2013accessid, slankas2013implementing}. However, text classification techniques were also employed to identify access decisions (i.e. allow or deny) \cite{heaps2021access, xia2022automated}, to identify access type (i.e. read, write, etc. ) \cite{heaps2021access} and to categorize similar subject and resource attributes to generate a common name for the attributes \cite{alohaly2018deep, alohaly2019towards, alohaly2019automated, xia2022automated}. 

In the extracted publications, the text classification was either done by rule-based techniques \cite{xiao2012automated, brodie2006empirical, brodie2005usable} or machine learning-based techniques \cite{slankas2012classifying, slankas2014relation, slankas2013access, slankas2013accessid, slankas2013implementing, heaps2021access, xia2022automated}. In the rule-based approach, the ACP sentences were identified by matching the syntactic and semantic patterns of the natural language sentence with the pre-defined patterns \cite{xiao2012automated}. For instance, Xiao et al. identified the 4 most common grammatical patterns that define a NLACP \cite{xiao2012automated} as shown in Table \ref{tab:xiao_patterns}. Using those patterns, they filtered out the NL sentences that do not match with any of the identified patterns (i.e. sentences that do not contain access control policies). On the other hand, machine learning (ML)-based algorithms were also utilized to classify NLACPs. In contrast to rule-based techniques, machine learning-based techniques learn common patterns in non-ACP as well as ACP sentences without hardcoded rules, from a given training set, and classify an unseen sentence based on the learned patterns. For example, Support Vector Machine (SVM) classifier that identifies the best hyperplane (i.e. decision boundary) that separates ACP from non-ACP sentences based on their learned features was used by Slankas et al. to identify NLACPs from a NL document \cite{slankas2014relation, slankas2012classifying, slankas2013access, slankas2013accessid}. 

% Support Vector Machine (SVM) identifies the best hyperplane (i.e. decision boundary) that separates ACP from non-ACP sentences based on the distances between the sentences from the training dataset \cite{slankas2013access, slankas2013accessid}. When a new sentence comes in, it will be assigned to either one of the sides of the hyperplane depending on its distance to the hyperplane (e.g. if the distance is positive, the sentence is an ACP and non-ACP otherwise). However, if a distance metric is involved in the sentence classification techniques as in SVM or k-NN, it was calculated in different ways in the extracted literature. For example,  Slankas et al. introduced an improved version of Levenshtein distance as the distance metric for k-NN \cite{slankas2013accessid, slankas2012classifying}. The improved metric calculates the number of transformations needed to convert one sentence into the other (edit distance) and use it as the measurement of the distance. Later, Narouei et al. adapted the same improved k-NN classifier for their research \cite{narouei2015automatic, narouei2018automatic, narouei2015towards}.


% SVM is a supervised ML algorithm that finds the best hyperplane dividing data points into classes. Naive Bayes is a probabilistic ML algorithm which classifies data points by calculating the probability for each class using Bayes' Theorem given the input features. k-NN is a supervised ML algorithm which works by finding the k nearest data points to a given test data point and predicting a class for the test data point based on the majority class of the nearest neighbours.

\begin{table}[]
    \centering
    \caption{Semantic patterns in Access Control Sentences identified by Xiao et al. \cite{xiao2012automated}}
    \label{tab:xiao_patterns}
    \begin{tabular}{ 
   >{\centering\arraybackslash}m{6cm} 
   >{\raggedright\arraybackslash}m{8.3cm}}
        \toprule
        {\textbf{Semantic pattern}} &  {\textbf{Example}}\\
        \midrule
          Modal Verb in Main Verb Group & An HCP\textsubscript{[subject]} \textbf{can view} \textsubscript{[action]} the patient’s account\textsubscript{[resource]}.\\
          
         \noalign{\vskip 4.5pt}
          Passive Voice followed by To-infinitive Phrase & An HCP\textsubscript{[subject]} \textbf{is disallowed to update} \textsubscript{[action]} patient’s account\textsubscript{[resource]}. \\
          \noalign{\vskip 4.5pt}

          Access Expression & An HCP\textsubscript{[subject]} \textbf{has read}\textsubscript{[action]} \textbf{access to} patient’s account\textsubscript{[resource]}. \\
          \noalign{\vskip 4.5pt}

          Ability Expression & An HCP\textsubscript{[subject]} \textbf{is able to read} \textsubscript{[action]} patient’s account \textsubscript{[resource]}. \\

         \bottomrule
         
    \end{tabular}
    
\end{table}

\begin{table}[]
    \centering
    \caption{Text classification techniques}
    \label{tab: classification}
    \begin{tabular}{ 
   >{\centering\arraybackslash}m{6cm} 
   >{\raggedright\arraybackslash}m{6cm}
   >{\raggedright\arraybackslash}m{2cm}}
   
        \toprule
        \textbf{Classification technique} &  \textbf{Classification task} & \textbf{References} \\
        \midrule
         Support Vector Machines (SVM) & ACP classification & \cite{slankas2013access, slankas2013accessid}\\
         \noalign{\vskip 3.5pt} 
         Naive Bayes & ACP classification & \cite{slankas2013access, narouei2017identification}\\
          & Policy component relation classification & \cite{slankas2014relation}\\
         \noalign{\vskip 3.5pt} 
         k-Nearest Neighbours (k-NN) & ACP classification & \cite{slankas2014relation, slankas2012classifying, slankas2013access, slankas2013accessid, narouei2015automatic, narouei2018automatic, narouei2015towards}\\
           & Policy attribute classification & \cite{alohaly2019automated} \\
         %   \noalign{\vskip 3.5pt} 
         % Density Based Spatial Clustering of Application with Noise (DBSCAN) & Policy attribute value clustering & \cite{alohaly2019automated} \\
         % \noalign{\vskip 3.5pt}
         % Ordering points to identify the clustering structure (OPTICS) & Policy attribute value clustering & \cite{xia2022automated} \\
         \noalign{\vskip 3.5pt}
         Decision Tree & Access decision classification & \cite{singru2020efficient} \\
         \noalign{\vskip 3.5pt} 
         Syntactic pattern matching & ACP classification & \cite{xiao2012automated, yang2021purext} \\
         \noalign{\vskip 4.5pt}
         Convolutional Neural Networks (CNN) & Policy attribute relation classification & \cite{alohaly2018deep, alohaly2019automated} \\
         \noalign{\vskip 3.5pt} 
         Long short term memory (LSTM) & ACP classification & \cite{narouei2017towards} \\
         \noalign{\vskip 3.5pt} 
         Transformers (BERT) & ACP classification and Access type classification & \cite{heaps2021access, xia2022automated} \\
         % \noalign{\vskip 3.5pt} 
         % Transformers (BERT) + Semantic Role Labelling (SRL) & ACP classification & \cite{xia2022automated} \\
         \bottomrule

         
    \end{tabular}
    
\end{table}

% When using clustering techniques such as as k-NN, a distance metric is used to identify the cluster d
% On a few occasions, the distance metric of the k-NN algorithm was modified when classifying access control policies, as the metric should be able to calculate the distance between sentences, instead of numerical values.

% Therefore, Slankas et al. introduced an improved version of Levenshtein distance as the distance metric for k-NN \cite{slankas2013accessid, slankas2012classifying}. The improved metric calculates the number of transformations needed to convert one sentence into the other (edit distance). Later Narouei et al. adapted the same improved k-NN classifier for their research \cite{narouei2015automatic, narouei2018automatic, narouei2015towards}. 
% Nevertheless, if k-NN alone was used to classify the sentences using a similarity threshold, Slankas et al. noticed that the F1 performance of the classification was 1.0 (no misclassifications), even though not all the sentences were classified \cite{slankas2012classifying}. Therefore, to improve the robustness of the classification system, Slankas et al. utilized multiple traditional ML classifiers for the classification task (Ensemble Classifier) \cite{slankas2013access, slankas2013accessid}. They used SVM and Naive Bayes together with k-NN to get the majority vote as the classification result to reduce overfitting. In machine learning, this technique is called "Bagging".   

Apart from the traditional machine learning-based classification techniques, neural network-based classification was also employed in the included literature. For instance, Alohaly et al. \cite{alohaly2018deep, alohaly2019automated} used a Convolutional Neural Network (CNN) to classify whether the identified subject and object attribute relations are valid or not. Furthermore, with the new developments of the NLP domain, Transformers \cite{vaswani2017attention} were also used on several occasions to carry out classification tasks related to access control policies \cite{heaps2021access, xia2022automated}. For example, Heaps et al. \cite{heaps2021access} utilized Bi-directional Encoder Representation for Transformers (BERT) \cite{devlin2018bert} to classify user stories as ACP, non-ACP (i.e. not an access control policy) and ambiguous as well as to classify their access type (i.e. read, write, etc.). All the identified text classification techniques and related references are shown in Table \ref{tab: classification}.
% Also, by utilizing BERT-based SRL, Xia et al. classified NLACPs based on their semantic features \cite{xia2022automated}. 
% each semantic role label sequences for each predicate of the NLACP, were first pruned to remove the non-ACP verbs based semantic roles. Then, they adopt CNN to generate the word level embeddings from BERT embeddings, for each word of the sentence. Finally, they classify the sentences as ACP and non-ACP after fusing the generated embeddings and the vectorised pruned semantic role labels. 

After identifying the ACP sentences from the NL documents, necessary components of the NL policy should be extracted to generate the machine-executable policy. Therefore, as the next step, information extraction was carried out.  

\textbf{Information Extraction} - Information extraction is the process of extracting structured information from unstructured or semi-structured data sources such as NL sentences and NL documents \cite{cui2018neural}. Table \ref{tab: ie} shows the information extraction techniques used in the previous literature with the associated references.

\begin{table}[]
    \centering
    \caption{Information (IE) techniques}
    \label{tab: ie}
    \begin{tabular}{ 
   >{\centering\arraybackslash}m{6cm} 
   >{\raggedright\arraybackslash}m{6cm}
   >{\raggedright\arraybackslash}m{2cm}}
   
        \toprule
        \textbf{Information extraction technique} &  \textbf{Extracted information} &  \textbf{References}  \\
        \midrule 
          Syntactic parsing & ACP component extraction & \cite{brodie2006empirical, xiao2012automated, vaniea2008evaluating, karat2006evaluating, reeder2007usability, brodie2005usable, slankas2013access, narouei2017identification, ye2016identify, yang2021purext, slankas2014relation, alohaly2019towards, tanoli2018towards, xia2022automated, shi2011controlled, fatema2016semi, inglesant2008expressions, vanbrabant2009federated, vanbrabant2011fine, turner2017proposed, shen2021using, basile2010ontology}\\
          \noalign{\vskip 1pt}
           & ACP attribute extraction & \cite{alohaly2018deep, alohaly2019automated, xia2022automated}\\
          \noalign{\vskip 4pt}
            % \hdashline
          Semantic Role Labeling (SRL) & ACP component extraction & \cite{xia2022automated, narouei2015automatic, narouei2018automatic, yang2021purext, narouei2017towards, narouei2015towards}\\
          \noalign{\vskip 1pt}
           & ACP attribute extraction & \cite{xia2022automated}\\
        \noalign{\vskip 4pt}
        % \hdashline
          Named Entity Recognition (NER) & ACP component extraction & \cite{ narouei2015automatic,narouei2015towards, heaps2021access, alohaly2019towards}\\
          \noalign{\vskip 1pt}
           & ACP attribute extraction & \cite{zhu2021unstructured}\\
           \noalign{\vskip 4pt}
        % \hdashline
          % Ontologies & ACP component extraction & \cite{shi2011controlled, inglesant2008expressions, fornara2016modeling, basile2010ontology, tanoli2018towards}\\
          % \noalign{\vskip 4.5pt}
            % \hdashline
          Other & ACP component extraction & \cite{amato2013semantic, alohaly2021hybrid, fornara2016modeling}\\
         \bottomrule
    \end{tabular}
\end{table} 

%  \begin{table}[]
%     \centering
%     \caption{Information (IE) techniques}
%     \label{tab: ie}
%     \begin{tabular}{ 
%    >{\centering\arraybackslash}m{6cm} 
%    >{\raggedright\arraybackslash}m{6cm}
%    >{\raggedright\arraybackslash}m{2cm}}
   
%         \toprule
%         \textbf{Information extraction technique} &  \textbf{Extracted information} &  \textbf{References}  \\
%         \midrule 
%           Shallow parsing & ACP component extraction & \cite{brodie2006empirical, xiao2012automated, vaniea2008evaluating, karat2006evaluating, reeder2007usability, brodie2005usable}\\
%           \noalign{\vskip 4.5pt}

%           Dependency parsing & ACP component extraction & \cite{slankas2013access, narouei2017identification, ye2016identify, yang2021purext, slankas2014relation, alohaly2019towards, tanoli2018towards, xia2022automated}\\
%           \noalign{\vskip 1pt}
%            & ACP attribute extraction & \cite{alohaly2018deep, alohaly2019automated, xia2022automated}\\
%            \noalign{\vskip 4.5pt}

%           Rule-based parsing & ACP component extraction & \cite{shi2011controlled, fatema2016semi, inglesant2008expressions, vanbrabant2009federated, vanbrabant2011fine, turner2017proposed, shen2021using}\\
%          \noalign{\vskip 4.5pt}

%           SRL & ACP component extraction & \cite{xia2022automated, narouei2015automatic, narouei2018automatic, yang2021purext, narouei2017towards, narouei2015towards}\\
%           \noalign{\vskip 1pt}
%            & ACP attribute extraction & \cite{xia2022automated}\\
%         \noalign{\vskip 4.5pt}

%           NER & ACP component extraction & \cite{ narouei2015automatic,narouei2015towards, heaps2021access, alohaly2019towards}\\
%           \noalign{\vskip 1pt}
%            & ACP attribute extraction & \cite{zhu2021unstructured}\\
%            \noalign{\vskip 4.5pt}

%           Ontologies & ACP component extraction & \cite{shi2011controlled, inglesant2008expressions, fornara2016modeling, basile2010ontology, tanoli2018towards}\\
%           \noalign{\vskip 4.5pt}
 
%           Other & ACP component extraction & \cite{amato2013semantic, alohaly2021hybrid}\\
%          \bottomrule
%     \end{tabular}
% \end{table}

Among the identified literature, the most prevalent technique used to extract information from NLACPs (48\%) is syntactic parsing. 
% performed using libraries including NLTK, SpaCy, CoreNLP, and Stanford dependency parser. 
Syntactic parsing is a method of analyzing the grammatical structure of a sentence. It identifies the syntactical relationships between words of a sentence and ultimately creates a structured representation of the sentence named "Parse tree". 
% Parse tree can further be simplified into an intermediate representation named Abstract Syntax Tree (AST), which was also used in the extracted literature to identify the policy components \cite{vanbrabant2009federated, vanbrabant2011fine}. 
There are 2 main syntactic parsing techniques that were utilized in policy component extraction studies: shallow parsing \cite{xiao2012automated, brodie2005usable, brodie2006empirical, vaniea2008evaluating, karat2006evaluating, reeder2007usability, perry2013modular} and dependency parsing \cite{alohaly2019automated, alohaly2018deep, slankas2012classifying, slankas2013access, slankas2013accessid, slankas2013implementing, slankas2014relation, yang2021purext, tanoli2018towards, ye2016identify, alohaly2019towards, narouei2017identification, xia2022automated}. 
% in NLP \cite{zhang2006exploring, culotta2004dependency, zelenko2003kernel}. 
% They are Constituency parsing \cite{pollard1994head}, and Dependency parsing \cite{covington2001fundamental}. Constituency parsing recursively breaks down a sentence into its constituent phrases \cite{zhang2020survey}. For instance, consider the sentence \emph{"He reads a file"}. In constituency parsing, \emph{reads a file} is a verb phrase (VP), which in turn contains a noun phrase (NP), \emph{a file}. However, constituency parsing is considered a complex, slow process and tends to struggle with ambiguities and incomplete sentences \cite{zhang2020survey}. Instead, in the access control policy generation domain, researchers used a partial parsing technique named 
Shallow parsing, or "Chunking" divides the sentence into constituents called "Chunks" according to the syntactic structure of the natural language sentence \cite{sha2003shallow}.
% In contrast to the constituency parsing, the chunks will not be further analyzed recursively. Therefore, in shallow parsing, depth of analysis and completeness are sacrificed for the efficiency and reliability. Generating chunks is done according to a predefined set of grammar depending on the task. 
In order to form "chunks" of NLACPs, grammar rules should be developed by considering a common sentence structure (i.e. template) of a NLACP \cite{brodie2006empirical}. For example, consider the following simple grammar rules. \texttt{NP: \{<JJ>?<NN>*\}, VP: \{<VB>\}, NP: \{<NP><POS><NP>\}}. After feeding the above rules to a shallow parser\footnote{There are shallow parsers provided by some popular NLP libraries such as NLTK, SpaCy and CoreNLP}, it will first create chunks by combining adjectives (JJ) and nouns (NN), and tag the chunks as noun phrases (NP). Then the shallow parser will tag verbs (VB) as a verb phrase. Finally, it will form chunks containing a noun phrase (NP) followed by a genitive marker (i.e. "'s") (POS) and another noun phrase (NP) to tag them as a noun phrase (NP). Using the aforementioned grammar rule the NLACP, \emph{"The doctor can read patient's record"} will be tagged as shown in Fig. \ref{fig:shallow_parser} and the policy components such as the subject, the action, and the resource can easily be extracted. Following the same procedure, Brodie et al. designed a set of grammar rules for the "SPARCLE policy workbench" that operate in order (sequentially) to add tags to the NLACPs indicating the places where policy components start and end. They used the cascaded structure to first extract the hard-to-extract components such as conditions, obligations, and purposes, and then to extract user categories, data categories, and finally actions \cite{brodie2006empirical}. However, to be able to extract components from shallow parsing, NLACPs should be written according to a specific template that was used to define grammar rules. For example, if the mentioned NLACP is written in a different structure such as \emph{"Patient's record can only be read by the doctor"}, the aforementioned grammar rules may not be able to parse the NLACP and identify the components.

\begin{figure*}[]
    \centering
    \includegraphics[height=3cm]{images/parser.png}
    \caption{Shallow parse tree generated using NLTK library for the sentence \emph{"The doctor can read patient's record"} according to the grammar rules \texttt{NP: \{<JJ>?<NN>*\}, VP: \{<VB>\}, NP: \{<NP><POS><NP>\}}. NP: Noun phrase, NN: Noun, JJ: Adjective, VP: Verb Phrase, VB: Verb in its base form, POS: genitive marker (i.e. "'s")}
    \label{fig:shallow_parser}
\end{figure*}



% On the other hand, dependency parsing focuses on extracting the dependent relationships between words of the sentence, rather than extracting phrases. Therefore, in contrast to the constituency and shallow parsing, the dependency tree is a directed graph containing words of the sentence as nodes, and the relationships between words as edges \cite{ambati2008dependency}. 
% Constituency, Shallow, and Dependency parse trees of the aforementioned NLACP example (i.e. \emph{"He reads a file"}) are shown in Fig. \ref{fig:parse}. 

% \begin{figure}[!ht]
% \centering
% \captionsetup[subfigure]{justification=centering}
% \subfloat[Constituency Parsing]{
%         \centering
%         \includegraphics[width=0.4\textwidth]{images/const.png}
%         \label{fig:const}
%     }
%     \hfill

%     \subfloat[Shallow Parsing]{
%         \includegraphics[width=0.4\textwidth]{images/shallow.png}
%         \label{fig:shallow}
%     }

%     \hfill
    
%     \subfloat[Dependency Parsing]{
%         \includegraphics[width=0.4\textwidth]{images/dep.png}
%         \label{fig:dep}
%     }
    
%     \vspace{0.5em}
%     \captionof{figure}{Parse trees of the sentence \emph{"He reads a file"}}
%     \label{fig:parse}
% \end{figure}

% On the other hand, relation extraction studies have empirically shown that the patterns derived from dependency parsing are more resilient to lexical inconsistencies compared to constituency parsing \cite{johansson2008dependency}. 
On the other hand, 23.1\% of the extracted publications utilized dependency parsing for the policy component/attributes extraction \cite{alohaly2019automated, alohaly2018deep, slankas2012classifying, slankas2013access, slankas2013accessid, slankas2013implementing, slankas2014relation, yang2021purext, tanoli2018towards, ye2016identify, alohaly2019towards, narouei2017identification, xia2022automated}. In contrast to shallow parsing, dependency parsing identifies the relationships between words in a sentence and generates a directed graph containing the tokens as the nodes and relationships as the edges. For instance, the dependency parse tree of the NLACP \emph{"The doctor can read patient's record"} is shown in Fig. \ref{fig:dep_parser}. According to the figure, between the subject, doctor, and the action, read has the nominal subject (nsubj) relationship. Furthermore, the direct object (dobj) relationship can be seen between the action and the resource, patient's record. 

\begin{figure*}[]
    \centering
    \includegraphics[height=2.5cm]{images/dep_parser.png}
    \caption{Dependency parse tree generated using SpaCy library for the sentence \emph{"The doctor can read patient's record"}. det: relationship between determiner (DT) and noun (NOUN), nsubj: relationship between the noun and verb (VERB), aux: relationship between auxiliary verb (AUX) and main verb, dobj: relationship between verb and object, poss: relationship between a noun and its possessive modifier, case: relationship between a noun and its case marker (PART).}
    \label{fig:dep_parser}
\end{figure*}

To identify the policy components in a NLACP, the most common dependency relationships between components should be identified first. Therefore, Slankas used the "bootstrapping" mechanism to identify different dependency relationships in NLACPs starting from known 10 seed patterns with 3 vertices (subject, operation, and resource) and expanded the pattern database with new patterns along the way \cite{slankas2014relation, slankas2013access}. All the known seed patterns were the same except the verb representing 10 different actions namely create, retrieve, update, delete, edit, view, modify, enter, choose, and select. The subject and the resource nodes were kept as wildcards to match and extract any nouns associated with the verb. After extracting subjects and resources using the seed patterns, they expanded their pattern database in 2 ways: (1) by extracting additional dependency patterns that contain the known subjects and resources, (2) by applying a series of transformations to the existing patterns (e.g. transforming the patterns in active voice into passive voice). The most common dependency patterns identified in ACP sentences by Slankas et al. \cite{slankas2014relation} are listed in the 1st column of Table \ref{tab: slankas_patterns}.
% In contrast to shallow parsing, patterns identified in dependency parsing are based on the \textbf{relationships} between the words of the sentence. Thus, the dependency patterns represent the relationships between policy components including subjects, operations, and resources as well as the relationships between attributes such as subject attributes, object attributes, and environment attributes. 
Moreover, Alohaly et al. report the 5 most common relations that encode subject-attributes and object-attributes of NLACPs in \cite{alohaly2019automated} (See column 2 and 3 of Table \ref{tab: slankas_patterns}). In contrast to Slankas et al. \cite{slankas2014relation, slankas2013access}, Alohaly et al. manually extracted the relationship patterns from their NLACP dataset. Nevertheless, it is important to note that the effectiveness of using a dependency parser for policy component extraction is solely dependent on the quality and quantity of the identified patterns in the pattern database. 

\begin{table}[]
    \centering
    \caption{Dependency patterns that encode relationships between the policy components (column 1), subject-attributes (column 2), and object-attributes (column 3) of Access Control Sentences. VB: verb, NN: noun, nsubj: nominal subject, dobj: direct object, nsubjpass: passive nominal subject, amod: adjectival modifier, prep: prepositional modifier, pobj: object of preposition}
    \label{tab: slankas_patterns}
    \begin{tabular}{ 
   >{\centering\arraybackslash}m{5cm} 
   >{\raggedright\arraybackslash}m{5cm}
   >{\raggedright\arraybackslash}m{4cm}}
        \toprule
        \textbf{Patterns between policy components \cite{slankas2014relation}} &  \textbf{Patterns between subject-attributes \cite{alohaly2019automated}} & \textbf{Patterns between object-attributes \cite{alohaly2019automated}}\\
        \midrule
          (VB root (NN nsubj) (NN dobj)) & nsubj, amod & dobj, amod\\
          
         \noalign{\vskip 4pt}
         % \hdashline

          (VB root (NN nsubjpass)) & nsubj, prep & pobj, amod \\
          \noalign{\vskip 4pt}
          % \hdashline

          (VB root (NN nsubj) (NN prep)) & nsubjpass, amod & dobj, prep\\
          \noalign{\vskip 4pt}
          % \hdashline

          (VB root (NN dobj)) & nsubj, compound & dobj, compound \\
          \noalign{\vskip 4pt}
          % \hdashline

          (VB root (NN prep\_\%)) & nsubj, ROOT, amod & nsubjpass, amod \\
          \bottomrule
    \end{tabular}
\end{table}

% Apart from the common parsing techniques discussed above, several other rule-based parsing techniques were also used in literature \cite{shen2021using, fatema2016semi, turner2017proposed, perry2013modular}. For example, Shen et al. \cite{shen2021using} utilized rule-based techniques such as keyword extraction and tag alignment to identify the syntactic features of NLACPs written in Chinese. In keyword extraction, several domain-related words were searched using a domain dictionary in NLACPs and extracted. It helps to divide the sentence into segments as there are no spaces between Chinese characters. Then the tag alignment was performed by combining keywords into chunks and extracting the desired attributes. 

% The database used to extract keywords can also be called a "Domain dictionary" as it contains the domain-related terms \cite{xiao2012automated}. Domain dictionaries were used in 13.5\% of the identified articles, for different objectives other than segmentation throughout the extracted articles. For example, Xiao et al. used domain dictionaries to associate the verbs of NLACP sentences with pre-defined semantic classes \cite{xia2022automated}, Xia et al. \cite{xia2022automated} used a dictionary containing non-ACP verbs to prune the semantic labels generated for NLACPs, Ye used a keyword database to classify service rules into different semantic categories \cite{ye2016identify}, and Alohaly et al. used a data dictionary to store the ACP attributes and their allowable values in \cite{alohaly2021hybrid}. 

Semantic Role Labeling (SRL) and Named Entity Recognition (NER)\cite{tjong-kim-sang-de-meulder-2003-introduction} are also popular information extraction techniques used in previous literature \cite{xia2022automated, heaps2021access, narouei2015towards, narouei2017towards, narouei2018automatic, yang2021purext, zhu2021unstructured}. SRL is used to analyze the meaning of the sentence by extracting its predicate-argument structure, determining "\emph{who did what to whom}", "\emph{when}", "\emph{where}", etc. \cite{shi2019simple}. Since SRL explicitly detects the subject (\emph{who}), action (\emph{what}), resource (\emph{whom}), as well as other environment attributes such as location (\emph{where}) and time (\emph{when}), previous literature extensively employed different semantic role labeling tools to extract policy components and attributes.
% The semantic role is the relationship between a predicate (verb or the verb phrase) and the words that denote the arguments or participants of the predicate. 
Some of them are SENNA (Semantic/Syntactic Extraction using a Neural Network Architecture) \cite{collobert2011natural}, neural network-based semantic role labeler used by Narouei et al. \cite{narouei2015automatic, narouei2015towards, narouei2017towards, narouei2018automatic}, SwiRL \cite{surdeanu2005semantic} used by Narouei et al. \cite{narouei2018automatic} and Yang et al. \cite{yang2021purext}, EasySRL \cite{lewis2015joint} used by Narouei et al. \cite{narouei2018automatic}, Mate-tools Semantic Role Labeler \cite{bjorkelund2009multilingual} used by Narouei et al. \cite{narouei2018automatic} and BERT-based SRL \cite{shi2019simple} used by Xia et al. \cite{xia2022automated}. 

% However, there are 2 main problems in using SRL to extract policy components. While SRL extracts most of the required policy components, it only extracts one argument from each type (e.g. ARG0, ARG1, ARGM-PRP, ARGM-ADV, etc.) for a given predicate. Therefore, all the users will not be extracted separately from policies that allow multiple users to do the same operation on a resource. For instance, BERT-based SRL by Shi et al. \cite{shi2019simple} identifies \emph{"The doctor and the nurse"} as the user (ARG0) in the policy \emph{"The doctor and the nurse can read patient's records."}. Secondly, SRL models were often trained to generate multiple outputs belonging to each predicate in the input sentence. In the above example BERT-based SRL model \cite{shi2019simple} outputs 2 sequences of labels related to the 2 predicates, \emph{can} and \emph{read}. Therefore, a pruning technique has to be employed to filter the unwanted predicate-based label sequences first, to extract policy components from the correct predicate-based output \cite{xia2022automated}. 



% For example, in the sentence \emph{"The doctor may read patient's records"}, the predicate is \emph{read} and the arguments are \emph{The doctor} and \emph{patient's record}. The semantic roles of the above sentence are shown in Fig. \ref{fig: srl}. 

% \begin{figure}[]
%   \centering
%     \includegraphics[width=1\linewidth]{images/srl.png}
%     \caption{Semantic roles of the sentence \emph{"The doctor may read patient's records"}.}
%     \label{fig: srl}
% \end{figure}
On the other hand, Named Entity Recognition (NER) is a NLP task that identifies the named entities of a given sentence. Therefore, several extracted publications used NER to extract entities related to access control domain such as subjects, actions, resources, etc. from NLACPs \cite{heaps2021access, zhu2021unstructured}. For example, Heaps et al. fine-tuned BERT language model \cite{devlin2018bert} using a dataset containing user stories \cite{dalpiaz2018pinpointing}, to extract such named entities to build access control policies \cite{heaps2021access}. They used the BIO-labeling technique to annotate each of the NLACP in the dataset.

% However, there is one major problem with using NER to identify policy components. When identifying the named entities such as subjects, actions, and resources, those entities do not show a relationship with each other. This is problematic when a single NLACP contains multiple policies. For instance, in the sentence \emph{"The doctor can read and write patient's record, but the nurse cannot write patient's records"}, named entities can be extracted as subjects: doctor, nurse, actions: read, write and resources: patient's record. Even though the recognized entities are correct, those entities do not say that the doctor is the one who can both read and write the patient's records, and the nurse can only read the patient's records. Therefore, someone can misinterpret the results as both the subjects can perform both the action on the resource. This property makes NER unsuitable for policy component extraction when multiple ACPs are present in the NL sentence unless the relationships between the entities are introduced to the process.


% To add the temporal information of words of the ACP sentence for attribute mining, Zhu et al. attached RoBERTa model with a BiLSTM (Bi-directional Long Short Term Memory) module with a CRF (Conditional Random Field) module to take the interdependence of the attributes into account.  
% Several extracted publications utilized different types of RNNs to improve their information extraction frameworks by sharing learned features across subsequent positions of the NLACP  \cite{zhu2021unstructured, xia2022automated, alohaly2019towards}. One such type is Long-Short Term Memory (LSTM) networks designed to avoid problems in RNNs such as vanishing and exploding gradients  \cite{hochreiter1997long}. However, both RNN and LSTM networks process the input sentence only in the forward direction (i.e. sequentially) allowing only to associate dependencies between words before, with the current word of the sentence. By improving the LSTM network architecture, so that it can capture the long-term dependencies between past and future words, Bi-directional LSTM (BiLSTM) was introduced. By taking advantage of the above improvement, Zhu et al. used a BiLSTM network together with a language model (RoBERTa) and CRF to mine ABAC attributes, while Alohaly et al. utilized BiLSTM network to identify the constraints in NL ABAC policies \cite{alohaly2019towards}. 

% Ontology-based approaches are also common in the previous literature to extract and represent information from ACPs in a structured format \cite{tanoli2018towards, fornara2016modeling, shi2011controlled, inglesant2008expressions, basile2010ontology}. An ontology is a structured set of concepts, relationships, instances, and axioms that are used to represent information in a particular domain in terms of objects, properties, and classes \cite{reyes2019ontology}. In order to develop ontologies, tools such as GATE \cite{cunningham2002gate} were used in the extracted articles together with an ontology language (e.g. OWL (Web Ontology Language)). For instance, Shi et al. \cite{shi2011controlled} and Inglesant et al. \cite{inglesant2008expressions} developed ontology-based interfaces with GATE/CLoNE software \cite{cunningham2002gate}, which allow the administrator to write access control policies in Controlled Natural Language (CNL). In the proposed software, upon providing the manually built ontology using OWL, it will be populated with the CNL-based access control policies as written by the administrator. However, manually developing an ontology is a time consuming task. Therefore, instead of manually generating the entire ontology at the beginning \cite{shi2011controlled, inglesant2008expressions}, Basile et al. used an ontology that expands by deriving new classes based on the previous levels of the ontology \cite{basile2010ontology}. They used the mentioned ontology-based approach to translate NL network policies to machine-executable policies mimicking the administrator without the mistakes \cite{basile2010ontology}.


% To parse the CNL policies, Shi et al. further developed a parser using GATE and  one  of  its  applications  called  CLOnE  (Controlled Language for Ontology Editing). 
% Finally, the ontology will be exported in a form of an access control language such as XACML or PERMIS. 
% Moreover, instead of generating the entire ontology manually, Basile et al. \cite{basile2010ontology} developed an "ontology reasoner" which expands the ontology by adding classes derived from the classes from previous levels of the ontology.

% Once the policy components and attributes were extracted, those information should be rearranged into machine-executable format to apply the policies into the target computer system. 

\textbf{Information Transformation} - After extracting the policy components and attributes, extracted information was transformed into an intermediate representation/machine executable format, in 38.5\% of the included publications. The most common transformation format among literature was XACML (eXtensible Access Control Markup Language), which was used in 21.2\% of the articles \cite{xia2022automated, turner2017proposed, amato2013semantic, slankas2012classifying, fatema2016semi, vanbrabant2011fine, brodie2005usable, vaniea2008evaluating, shi2011controlled, karat2006evaluating, brodie2006empirical}. Apart from XACML representation of the policy, other XML-based representations such as PERMIS (Policy Enforcement through Role-based access control Mechanisms Implementation and Specification) \cite{inglesant2008expressions, shi2011controlled}, and EPAL (Enterprise Privacy Authorization Language) \cite{brodie2005usable, brodie2006empirical, vaniea2008evaluating, karat2006evaluating} were also employed in the extracted publications. However, if the policy generation pipeline outputs the generated policies in a specific policy language, its flexibility is reduced. Because the pipeline is not compatible with a system that uses a different policy language. Therefore, several publications propose policy generation frameworks that output an intermediate representation in terms of an ontology, without being limited to a specific policy language \cite{shi2011controlled, inglesant2008expressions, basile2010ontology, fornara2016modeling, tanoli2018towards}. 

% An ontology is a structured set of concepts, relationships, instances, and axioms that are used to represent information in a particular domain in terms of objects, properties, and classes \cite{reyes2019ontology}. In order to develop ontologies, tools such as GATE \cite{cunningham2002gate} were used in the extracted articles together with an ontology language (e.g. OWL (Web Ontology Language)). For instance, Shi et al. \cite{shi2011controlled} and Inglesant et al. \cite{inglesant2008expressions} provide a manually developed ontology in OWL. Once the input controlled natural language-based policies were parsed, the ontology will be populated and exported as the output. However manual ontology development is a laborious task. Therefore, instead of manually generating the entire ontology at the beginning \cite{shi2011controlled, inglesant2008expressions}, Basile et al. used an ontology that expands by deriving new classes based on the previous levels of the ontology \cite{basile2010ontology}.

Once the policies are formed in a structured format, those policies should be evaluated next to ensure their correctness before applying them to the system.


% The aforementioned representation formats are called "Policy languages" as they are used to specify, execute and enforce policies in machines (e.g. Computers). In contrast to the above policy languages, frameworks such as RDF (Resource Description Format) which is used to model and share data by describing resources as triplets (subject, predicate, and object) \cite{ye2016identify, amato2013semantic, shi2011controlled} as well as query languages such as SPARQL (SPARQL Protocol and RDF Query Language) which can be used to query and enforce RDF-based policies \cite{fornara2016modeling} can also be found in literature as a medium for information transformation. 

\textbf{Evaluation} - Evaluation metrics are used to assess the quality of the ML/NLP model by comparing its predictions with the ground truth, known as the "gold standard". Among many possible evaluation metrics, precision, recall, and F1 score were widely adopted in the extracted literature mainly when identifying the ACPs from NL documents and extracting policy components \cite{xiao2012automated, xia2022automated, slankas2013access, slankas2013accessid, slankas2012classifying, slankas2014relation, narouei2015towards, narouei2017towards, narouei2018automatic, narouei2017identification, alohaly2018deep, alohaly2019automated, alohaly2019towards, heaps2021access, brodie2006empirical, shen2021using, yang2021purext, zhu2021unstructured}. 

% Precision measures the proportion of true positives ($TP$) with respect to the total positive instances ($TP + FP$) as classified by the model. On the other hand, recall or "sensitivity" calculates the proportion of true positives ($TP$) that were correctly identified by the model (i.e. with respect to the total true positives ($TP$) and false negatives ($FN$)). Once the precision and recall are calculated F1 score, which is a single metric that balances both precision and recall can be derived. The above metrics can be calculated as follows.

% \begin{equation}
%     \label{eq:prec}
%     Precision\ (P) = \frac{TP}{TP + FP}
% \end{equation}

% \begin{equation}
%     \label{eq:rec}
%     Recall\ (R) = \frac{TP}{TP + FN}
% \end{equation}

% Using the equations (\ref{eq:prec}) and (\ref{eq:rec}),

% \begin{equation}
%     \label{eq:f1}
%     F1\ Score = \frac{2PR}{P + R}
% \end{equation}

Apart from the F1 score, Singru et al. used the accuracy metric to evaluate their model trained to classify the access decision according to the following formula \cite{singru2020efficient}. Here, $TP$, $TN$, $FP$ and $FN$ are the number of true positives, true negatives, false positives and false negatives respectively. 

\begin{equation}
    Accuracy = TP + \frac{TN}{TP + TN + FP + FN}
\end{equation}

\textbf{Datasets} - Datasets are of paramount importance in ML/NLP since the results and performance of the final model depend on the quality, quantity, annotations as well as completeness of the datasets. Especially, when it comes to a domain-specific learning task such as access control policy generation using NLP-based techniques. Even though, 32.7\% of the extracted studies have mentioned the details of the datasets that they used, most of them did not make the datasets public (mostly due to the confidentiality of such information). For instance, Naruoei et al. collected over 430 policy documents from the university policy office and health science center resulting in 21000 sentences, and annotated 2660 sentences containing 1460 ACP sentences and 1200 non-ACP sentences \cite{narouei2017towards}. However, the dataset is not publicly available.  

Nevertheless, we managed to find one dataset which is widely used among the extracted literature including \cite{narouei2015automatic, narouei2017towards, alohaly2016better,alohaly2018deep,alohaly2019automated,alohaly2019towards}, introduced by Slankas et al. in \cite{slankas2014relation}. The dataset contains 2477 sentences from multiple real-world systems such as health care data from iTrust \cite{meneely2012appendix}, educational data from IBM course registration system, conference management data from CyberChair, and the Collected ACP data from \cite{xiao2012automated}. Detailed information about the dataset is shown in Table \ref{tab: dataset}.

\begin{table}[]
    \centering
    \caption{Statistics of the dataset compiled by Slankas et al. \cite{slankas2014relation}}
    \label{tab: dataset}
    \begin{tabular}{ 
   >{\centering\arraybackslash}m{4.5cm} 
   >{\centering\arraybackslash}m{3cm}
   >{\centering\arraybackslash}m{3cm}
   >{\centering\arraybackslash}m{3cm}}
        \toprule
        \textbf{Data source} &  \textbf{Total sentences} & \textbf{ACP sentences} &  \textbf{non-ACP sentences}\\
        \midrule
          iTrust & 1631 & 967 & 664\\
          \noalign{\vskip 2pt}
          IBM Course Management (IBMCM) & 401 & 168 & 233\\
          \noalign{\vskip 2pt}
          CyberChair (CC) & 303 & 140 & 163\\
          \noalign{\vskip 2pt}
          CollectedACP (CACP) \cite{xiao2012automated} & 142 & 114 & 28\\
          \noalign{\vskip 2pt}
          \midrule
          \textbf{Total sentences} & 2477 & 1389 & 1088\\
          \noalign{\vskip 2pt}
          \textbf{Proportions} & - & 56\% & 44\%\\
          \bottomrule
    \end{tabular}
\end{table}

Another dataset was reported by Heaps et al. who proposed a framework to classify and extract policy components from user stories \cite{heaps2021access}. The dataset was developed by Dalpiaz et al. \cite{dalpiaz2018pinpointing} containing Over 1600 user stories from 21 web applications. However, the dataset was not annotated. 

\subsection{\rqtwo\ (RQ2)}
\label{subsec: limit_all}

According to the thematic analysis we conducted in Section \ref{subsubsec: data_analysis}, we identified several limitations/research gaps in the existing automated configuration tools we discussed in the last section. In this section, we point out several limitations in both GUI-based and NLP-based policy configuration tools, that will drive future research. 

\subsubsection{Limitations of graphical policy authoring and visualization interfaces}
\label{subsubsec:limit_gui}

Despite guiding the administrator to write and visualize access control policies manually, graphical policy authoring and visualization tools have their own limitations that hinder their effectiveness in accurate policy authoring and visualization. 

\textbf{Inability to write or visualize complex access control policies} - Access control policies may become complex when there are many different users, operations, and resources to manage in an organization. For instance, in a large organization with several departments, each department may have different access requirements for various users, systems, applications, and data. In such scenarios, defining access control policies for each user, resource, and operation can be complex as one policy may contain multiple users, resources, and operations as well as multiple purposes, obligations, and conditions.

As we noticed, more than 40\% of the proposed GUIs for access control authoring and visualization cannot handle such complex access control scenarios including \cite{reeder2008expandable, reeder2011more, vaniea2008access, morisset2018building, morisset2018visabac, brostoff2005r, bertard2020using, maxion2005improving, cao2006intentional}. For instance, as a policy authoring and visualization tool, Reeder's "Expandable Grids" interface does not support conditions, purposes or obligations to be included in the policy \cite{reeder2008expandable, reeder2011more}. Furthermore, connections between the nodes in different layers (i.e. Users, Roles and Loops) of the layered graph proposed by Bertard et al. \cite{bertard2020using} will be hard to distinguish clearly when there are many roles associated with users that perform actions on many resources at the same time as highlighted in Fig. \ref{fig: sugiyama}. This makes it challenging for the administrator to understand policies and ensure it is properly configured. 

\begin{figure}[]
  \centering
    \includegraphics[height=6.5cm]{images/sugiyama.png}
    \caption{Layered graph proposed by Bertard et al. to visualize access control policies. The red dotted box shows the connections that connect roles and loops (i.e. resources) that are harder to distinguish when multiple roles have permission to perform operations on multiple resources.}
    \label{fig: sugiyama}
\end{figure}
% Furthermore, modifying a complex policy using a GUI-based tool can also be difficult. Even a small modification or exception can cause unintended consequences such as allowing unauthorized access. A good example of a such scenario can be found in the user study conducted based on the "Expandable Grid" interface \cite{reeder2008expandable, reeder2011more}. In the aforementioned study, at one point participants had to restrict access for a user (U) in a group (G) to read a particular document. Later, they also had to modify the policy by allowing all the other members (except U) of the same group (G) to read the same document. Since the GUI semantics did not support such scenarios (deny-precedence), the participants ended up allowing all the members (including U) of the group (G) to read the document. 
 
\textbf{Lack of flexibility} - Graphical policy authoring tools often provide a pre-defined set of options or templates to define access control policies. Therefore, the ability to customize access control policies or policy structures according to specific use cases is limited. This limitation might be particularly problematic for organizations with unique access requirements, which are not covered by the pre-defined options. For instance, graphical policy authoring tools sometimes provide a specific set of templates that are specifically designed for a particular field. Turner introduced a GUI with a pre-defined template that suit for business rules \cite{turner2017proposed} while Rosa et al. proposed templates for the health care domain \cite{rosa2020parser}. However, the above pre-defined templates cannot be customized according to the unique access requirements of any other  type of organization. 
% Moreover, the supported policy structures cannot be customized without harming the policy parsing accuracy \cite{shi2011controlled, rosa2020parser, inglesant2008expressions, brodie2005usable, karat2006evaluating, vaniea2008evaluating, reeder2007usability}.
Therefore, it restricts the administrators to use the pre-defined templates despite the complexity and uniqueness of the policy requirement, resulting incomplete access control policies causing access control configuration failures \cite{inglesant2008expressions, brostoff2005r}.  

\textbf{Inconsistent interpretations} - GUI features, naming conventions as well as the visual representation of the access policies may not always be clear or intuitive to all users/administrators. Different administrators might interpret the same feature or the visual access control representation differently leading to inconsistencies in policy configuration. In fact, more than 20\% of the identified articles on GUI-based tools have potential issues directly or indirectly related to such inconsistent interpretations \cite{brostoff2005r, morisset2018building, morisset2018visabac, johnson2010optimizing, johnson2010usable}. 

For example, the same GUI feature can be interpreted differently by different administrators depending on their level of technical expertise, and their understanding of access control concepts. For example, in their usability trial study on a RBAC policy writing tool, Brostoff et al. made several interesting observations \cite{brostoff2005r}. They observed that non of the participants understand the label "SOA" (Source of Authority), 2 of the participants do not know about the word "RBAC" and some other participants misinterpreted SOA and RBAC when developing policies. Also, they found out that the unique naming convention they used for buttons was less intuitive for many inexperienced users/administrators. 
% They further found out the use of "Exclude button" was prone to misinterpretations as some users tried to use the button to exclude a newly defined subject in a system that denies all access except that which has been explicitly allowed. 

Furthermore, the use of colors and line styles to represent different operations and permission decisions in policy visualization techniques can easily be misinterpreted. For example, since the line styles used in VisABAC interface \cite{morisset2018building, morisset2018visabac} to denote operations "Deny Unless Permit (DUP)" and "Permit Unless Deny (PUD)" look almost similar in the interface (as shown in Fig. \ref{fig: visabac}), the administrator can wrongly identify them when dealing with policies containing many rules. This can result in confusion and misunderstandings when different users try to interpret the same policy as mentioned in \cite{bauer2009real}. 

\begin{figure}[]
  \centering
    \includegraphics[height=1.7cm]{images/visabac.png}
    \caption{Line conventions used by VisABAC to represent operations (a) Deny overrides (b) Permit overrides (c) Deny unless permit (d) Permit unless deny (e) First applicable (f) Only one applicable \cite{morisset2018building, morisset2018visabac}}
    \label{fig: visabac}
\end{figure}

\subsubsection{Limitations of NL-based policy configuration}
\label{subsubsec:limit_nlp}

As a result of the thematic analysis, we also found several noteworthy limitations of the existing NLP-based policy generation pipelines.

\textbf{Inability to handle ambiguities in NL policies} - Natural language access control policies are often abstract and ambiguous \cite{xiao2012automated}. Therefore, in order to identify and extract necessary policy components, the utilized NLP/ML algorithm should be capable of handling such ambiguous and abstract policies. However, more than 50\% of the publications employed syntactic parsing techniques to identify ACPs and extract their components  \cite{slankas2012classifying, slankas2013access, slankas2013accessid, slankas2014relation, xiao2012automated, brodie2005usable, brodie2006empirical, vaniea2008evaluating, karat2006evaluating, reeder2007usability}, which are limited in their ability to handle ambiguities \cite{manning1999foundations}. 
% For example, in the sentence \emph{"Administrators author access policies"}, dependency parsers often identify \emph{author} as a noun, instead of the verb of the sentence. 

% Furthermore, ontologies were also used to represent access control policies by defining the relationships between the policies in terms of pre-defined classes \cite{shi2011controlled, inglesant2008expressions}. Since the ontology was pre-defined expecting a specific structure from the NLACP, it will fail to parse and populate the ontology if an ambiguous or abstract policy was provided. For example, as Shi et al. mentioned, if the policy sentence is not clearly understandable according to their pre-defined semantics, the whole policy will be dropped \cite{shi2011controlled}.   

\textbf{Lack of flexibility} - In order to avoid the ambiguities of unconstrained natural language-based access ACPs, more than 28\% of the identified publications have used CNL-based policy authoring to write policies in NL including \cite{shi2011controlled, inglesant2008expressions, brodie2005usable, brodie2006empirical, karat2006evaluating, reeder2007usability, shen2021using, fatema2016semi, vanbrabant2009federated, vanbrabant2011fine}. CNLs are designed to be restrictive and precise, which can be helpful in preventing ambiguity and ensuring that policies are interpreted consistently \cite{wyner2009controlled}. However, this same restriction can limit the ability to express complex policies or make changes to existing policies. Brodie et al. restrict the user to follow only 2 semantic structures to write the policy \cite{brodie2006empirical}, while Shi et al. provided 5 semantic structures \cite{shi2011controlled} to write policies to avoid parsing failures. These restrictions limit the ability to express complex policies that require more nuanced or context-specific interpretations \cite{inglesant2008expressions}. 

% Due to the lack of flexibility of existing NL-based policy generation methods, several other challenges such as lack of generalization can also arise. Lack of generalization is the inability to adapt the same framework to configure policies in different domains. For example, Rosa et al. \cite{rosa2020parser} developed a parser to extract information from access control policies in the healthcare domain, written according to a specific template structure (i.e. sentence structure). Also, Turner introduced an ABAC policy generation tool based on a template related to business rules to be parsed using context-free grammars (CFG) in \cite{turner2017proposed}. However, since the above tools were developed for a specific use case/domain, while they lack of flexibility, they also cannot be generalized. 

\textbf{Lack of reliability} -  NLP-based policy generation frameworks were developed to operate with minimum human supervision \cite{heaps2021access}. Therefore, the policy generation pipelines should be reliable enough to generate machine-executable policies without the presence of the system administrator. However, in this SLR we identified several reasons that make the existing NLP-based automated policy generation frameworks less reliable (i.e. less accurate). 

One of the main reasons for low reliability is the insufficient coverage of different NLACP sentence structures by the rule-based parsing techniques used in previous literature. Being the most common information extraction technique in the identified articles, Rule-based parsers such as shallow parsers rely on pre-defined rules and patterns to parse and identify NLACPs \cite{brodie2006empirical, brodie2005usable, xiao2012automated}. However, it is challenging to create rules or identify patterns that cover all possible NLACP sentence structures that may contain policy components in different places and in different order. For example, Text2Policy \cite{xiao2012automated} which uses a shallow parser, can only identify ACPs that match with one of 4 sentence structures they defined (Table \ref{tab: slankas_patterns}). However, only 34.4\% of the sentences in the dataset used by Slankas et al. \cite{slankas2014relation} (Table \ref{tab: dataset}) agree with those 4 rules leaving the rest of the ACPs undetected, resulting in low ACP identification accuracy. 

To avoid using hard-coded pre-defined rules that do not cover every NLACP, deep learning-based models have been employed in some of the extracted publications that can identify patterns without having explicit rules \cite{narouei2015automatic, narouei2018automatic, yang2021purext, narouei2017towards, narouei2015towards}. However, the reliability of such deep learning-based models barely reaches the level of performance of the rule-based approaches. On the one hand, deep-learning models such as SRL models were not fine-tuned using domain-related access control data \cite{narouei2018automatic, alohaly2019automated, xia2022automated}. Because of that not only the model may not correctly identify policy components lowering the recall value but also the model will identify wrong subjects and resources related to non-access control predicates/actions such as 'can', 'have', 'is', 'become', etc. lowering the precision \cite{xia2022automated}. In the end, low precision and recall result in a low F1 score.
On the other hand, the components extracted by deep learning-based techniques lack granularity. For example, consider the following hypothetical access control policy (P). 

P: \emph{The pediatrician can read the patient's height and weight to prescribe medicine, if the patient's age is greater than or equal to 21.}

% P2: \emph{However he cannot prescribe medicine if the patient's age is greater than or equal to 21.}

If correctly identified, the extracted policy components of the above policy should look as follows. 

P: [\{pediatrician, read, patient\_height, none, prescribe medicine, allow\}, \{pediatrician, read, patient\_weight, patient\_age $\geq$ 21, prescribe medicine, allow\}]\footnote{P is structured according to the template \{subject, action, resource, condition, purpose, decision\}}

% P2: [\{pediatrician, prescribe, medicine, patient\_age $\geq$ 21, none, deny\}]

As shown above, if the information extraction output is granular enough, it should contain 2 sets of policy components corresponding to each of the 2 resources. However, most of the existing approaches fail to identify the two resources in P separately, instead \emph{patient's height and weight} will be identified as a single resource \cite{narouei2015automatic, xia2022automated, narouei2015towards, yang2021purext}. For instance, SRL-based approaches \cite{xia2022automated, narouei2015automatic, narouei2018automatic, yang2021purext, narouei2017towards, narouei2015towards}) can only identify one argument from each type (e.g. ARG0, ARG1, VERB, etc.) for a given predicate/action. Therefore, for the VERB \emph{read}, the SRL-based approach will identify \emph{pediatrician} as ARG0 and \emph{patient's height and weight} as ARG1. Thus the limited granularity. Therefore, to improve the granularity, a separate technique such as dependency parsing \cite{xia2022automated} or NER \cite{narouei2015towards} should be used together with SRL to separate the arguments into single entities. 

Nevertheless, existing approaches also often overlook important policy components, such as purposes, conditions, and obligations, when generating policies, resulting in limited expressiveness of the policy. For instance, in the above example, P contains a purpose, \emph{prescribe medicine}, a condition, \emph{patient's age is greater than or equal 21}, which are important to the context of the access control policy \cite{brodie2006empirical, brodie2005usable, karat2006evaluating, vaniea2008evaluating, reeder2007usability}. However, most of the policy component extraction techniques neglect those components \cite{xiao2012automated, slankas2014relation, slankas2012classifying, alohaly2019automated, xia2022automated, heaps2021access}. 

% In terms of the relationships between the policies, the policy extraction algorithm should identify that \emph{he} in P2 refers to the subject of P1, pediatrician (inter-relationship between P1 and P2). It is called "co-reference resolution" \cite{soon2001machine} or "anaphora resolution" \cite{kennedy1996anaphora}. However, none of the extracted publications attempted to extract such relationships between policies/rules. 

% However, none of the developed NLP frameworks are able to evaluate the purposes and conditions to be included in the machine-executable policy. For example, in R2, the condition \emph{patient's age is greater than 21} can be evaluated as $patient\_age \geq 21 $.
% Therefore, further investigations should be conducted to identify purposes, conditions as well as obligations for the sake of the completeness and granularity of the access control policy.  


\textbf{Lack of domain-related data} - Reliability and performance of the ML/NLP models heavily depend on the quality of the domain-related data. However, as many studies mentioned, the access control policy domain suffers from a scarcity of publicly available annotated datasets \cite{narouei2017towards, narouei2018automatic, narouei2017identification, alohaly2019automated, xia2022automated, yang2021purext, nobi2022machine}. Even if there are only 2 related datasets \cite{slankas2014relation, dalpiaz2018pinpointing}, the amount of data, the quality of the data, and the fact that annotations are either unavailable \cite{dalpiaz2018pinpointing} or incorrect \cite{slankas2014relation}, make it difficult to use them for fine-tuning deep learning models \cite{xia2022automated}. 
% Therefore the attention of the research community should be paid to developing a quality dataset with annotations or expanding the dataset by using augmentation and re-annotation techniques. 




==> Sections/misc.tex <==
NL-based access control policy generation process involves 2 crucial steps that use ML/NLP algorithms. They are the ACP classification (Text classification) step and the ACP component extraction (Information extraction) step. The accuracy of the final machine executable output will mainly depend on the reliability of the above 2 steps. However, the reliability and the accuracy measured according to the evaluation metrics we discussed earlier revealed that the ML/NLP algorithms used are prone to a significant amount of false positives and true negatives, which decrease the reliability of the final output.



\begin{enumerate}
    \item GUI tools focusing on policy authoring, such as text editors  \cite{stepien2009non, stepien2014non, zurko1999user, brodie2005usable, brodie2006empirical, brostoff2005r, reeder2007usability, vaniea2008evaluating, inglesant2008expressions, shi2011controlled, karat2006evaluating} and template-based authoring tools \cite{johnson2010optimizing, johnson2010usable, turner2017proposed, rosa2020parser}. 

    \item GUI tools focusing on policy visualization, such as graph-based policy visualization tools \cite{morisset2018visabac, morisset2018building, bertard2020using, heaps2021access}.

    \item GUI tools designed for both authoring and visualization such as access matrices-based tools \cite{reeder2008expandable, reeder2011more, vaniea2008access, cao2006intentional, maxion2005improving, reinhardt2021visual}.
\end{enumerate}


\subsection{Natural Language Processing (NLP)}
\label{subsec: nlp}

Natural Language Processing (NLP) is a branch of Artificial Intelligence (AI), that focuses on the interaction between human languages and computers. It involves the development of algorithms and techniques that enable computers to learn, understand and generate human language content \cite{hirschberg2015advances}. 
% Early computational techniques focused on statistical and symbolic NLP which were used to develop basic technologies such as machine translation, speech recognition, and speech synthesis. However, 
NLP has become increasingly important in recent years due to the explosion of digital content and the need to extract insights from unstructured data sources such as text, audio, and video. In order to cater to those growing needs, advanced NLP techniques were introduced starting from the neural language model \cite{bengio2000neural}, multi-task learning \cite{collobert2008unified}, word embeddings \cite{mikolov2013efficient}, sequence-to-sequence learning \cite{sutskever2014sequence}, attention \cite{bahdanau2014neural} to transformers \cite{vaswani2017attention}. 
% Based on the above techniques, NLP has come a long way. As evidence, the recent development of ChatGPT based on the InstructGPT \cite{ouyang2022training} and GPT-4 by OpenAI\footnote{https://openai.com}, which are large language models (LLMs) that show human-like understanding, can be mentioned. These models are based on the transformer architecture and have achieved state-of-the-art performance on a wide range of NLP tasks, including language modeling, machine translation, and question-answering. They are trained on massive amounts of text data and can generate human-like responses to natural language input, making them a promising technology for conversational AI applications.

Many natural language processing (NLP) and machine learning (ML) libraries were developed over the years that helped significantly to this development of advanced NLP models. Some of the popular NLP/ML libraries are Huggingface Transformers \cite{wolf2019huggingface}, NLTK\footnote{https://www.nltk.org/}, CoreNLP\footnote{https://stanfordnlp.github.io/CoreNLP/}, Spacy\footnote{https://spacy.io/} and Gensim\footnote{https://radimrehurek.com/gensim/}, TensorFlow\footnote{https://www.tensorflow.org}, Keras\footnote{https://keras.io}, and Pytorch\footnote{https://pytorch.org}. The aforementioned libraries not only speed up the development of advanced NLP models such as GPT-4 but also provide building blocks for researchers to build their own NLP pipelines. For example, access control policy generation using natural language is not a standard NLP task. However, previous research attempted to do it by combining multiple standard NLP/ML tasks with domain-specific pre and post-processing techniques. 

\subsubsection{Tokenization}

Tokenization is splitting a text into sentences, words, sub-words, or characters. Sentence-based tokenization is done by splitting sentences using delimiters such as ``.". Sentences are further divided into words using spaces or punctuation according to some pre-defined rules by a word-based tokenizer. Spacy and Moses\footnote{http://www2.statmt.org/moses/?n=Development.GetStarted} are such popular word-based tokenizers. For instance, the sentence \emph{``This is a word-based tokenizer"} will be tokenized into [``This", ``is", ``a", ``word", ``-", ``based", ``tokenizer"]. Since word-based tokenizers generate a large vocabulary and neglect the coherence between the words with similar meanings such as \emph{dog} and \emph{dogs}, character and sub-word-based tokenizers were introduced. Even though splitting a word into characters reduces the complexity and memory usage, it makes it much harder for the NLP algorithm to learn meaningful input representations. Therefore, sub-word-based tokenizers will not split frequently used words into smaller sub-words, but the words will be decomposed into meaningful sub-words if they are used rarely within the corpus. For instance, the word \emph{``annoyingly"} will be considered rare and divided into 2 sub-words \emph{``annoying"} and \emph{``ly"}. There are popular sub-words tokenization algorithms such as Byte Pair Encoding (BPE) \cite{sennrich2015neural}, WordPiece \cite{song2020fast} and SentencePiece \cite{kudo2018sentencepiece}, which are employed by modern NLP algorithms. Finally, the tokenizer converts the words, characters and sub-words into unique integers according to a lookup table. 

\subsubsection{Stemming and Lemmatization}

Stemming and lemmatization are the processes of reducing a word to its stem/ root/ base word \cite{khyani2021interpretation}. For instance, words such as \emph{``liked"}, \emph{``likes"}, \emph{``likely"} can be reduced to the root word \emph{``like"}. Even though both stemming and lemmatization are used for the same task, lemmatization is more complex than stemming. Lemmatization analyses the text morphologically using a dictionary to produce a meaningful stem/ root word while stemming generates the root word by removing suffixes or prefixes from the word \cite{khyani2021interpretation}. To understand the difference, consider the word \emph{``Caring"}. Lemmatizing the word will return \emph{``Care"}, which is semantically related to \emph{``Caring"}. However, stemming the word \emph{``Caring"} will return \emph{``Car"}, which has a completely different meaning from the original word. 

\subsubsection{Stop-word removal}

In this preprocessing technique, words that occur commonly in the corpus such as articles, prepositions, pronouns, conjunctions, etc. will be removed. By removing these words, the low-level information in a sentence will be removed by allowing the NLP algorithm to focus more on the important information. In most NLP applications, stop-word removal will not have negative consequences \cite{hardeniya2016natural}. 

\subsubsection{Part-Of-Speech (POS) Tagging}

POS tagging, in other words, grammatical tagging is used to assign each word of a text the proper syntactic tag in its context of appearance \cite{chiche2022part}. Manually tagging a sentence with syntactic tags is a tedious, laborious, and expensive task. Therefore, rule-based as well as machine learning-based POS taggers were introduced. NLTK, SpaCy, and CoreNLP libraries provide such POS taggers. For instance, the sentence \emph{``And now for something completely different"} will be tagged in NLTK as,\emph{``[('And', 'CC'), ('now', 'RB'), ('for', 'IN'), ('something', 'NN'), ('completely', 'RB'), ('different', 'JJ')]"}. Note that \emph{And} is CC, a coordinating conjunction; \emph{now} and \emph{completely} are RB or adverbs; \emph{for} is IN, a preposition; \emph{something} is NN, a noun; and \emph{different} is JJ, an adjective. \cite{nltk}.





However, surprisingly, only 12.5\% (2 \cite{heaps2021access, xia2022automated}) of the extracted publication published in or after 2018 (16) attempted to employ transformers (which was introduced in 2017 by Vaswani et al. \cite{vaswani2017attention}) for access control policy generation. Both of the publications are based on BERT \cite{devlin2018bert}, a transformer-based LM that was introduced in 2018. Furthermore, non of the extracted articles views that policy generation as a sequence-to-sequence (seq2seq) task, which generates the machine executable policy directly in a format such as XACML for a given NLACP without extracting components and transforming them separately. Not only it removes many post-processing and decision-making tasks such as choosing the correct predicate/action and argument relationship \cite{xia2022automated}, but also it avoids using multiple LMs sequentially to carry out sub-tasks in policy generation such as ACP classification, access type classification, etc. \cite{heaps2021access}, which increases the efficiency of policy generation. It can be done by supervised fine-tuning of decoder-only, encoder-decoder, or generative LMs such as GPT-2, GPT3, T5, BART, etc. that generate a textual output. Therefore \textbf{utilizing the capabilities of transformer-based architectures, especially decoder-only, encoder-decoder, and generative transformer-based LMs, and LLMs} by employing the techniques we described in Section \ref{sec:discussion} for access control policy generation can be explored in future research. As another gap in the reviewed literature, we observed that not only many studies did not attempt to extract "complex parts of the rule" such as purposes, conditions, and obligations \cite{brodie2006empirical}, but also none of the previous research evaluated them so that they are machine-understandable. For example, if the NLACP is \emph{"The doctor can treat the patient if the patient's age is 30 or higher"}, the condition \emph{"patient's age is 30 or higher"} can be evaluated as $patient\_age \geq 30$. This condition could act as a constraint that has to be checked before granting access. Therefore, \textbf{improving and developing policy generation models that can generate machine-executable policies with more complexity and granularity} can be another future research direction. 

By looking at the developed NLP-based access control policy generation techniques, it is evident that a ML/NLP model alone cannot reliably generate machine-executable access control policies without the administrator's supervision. Especially when the models trained on insufficient and less-quality datasets with low accuracy values are involved \cite{xia2022automated, heaps2021access, narouei2018automatic, narouei2017towards, narouei2015automatic}. For instance, Heaps et al. reported that their BERT-based policy component extraction model falsely identified "admitted" as a user, as it is close to the word "administrator" \cite{heaps2021access}. If such false positives were applied blindly without correcting them, they could result in incorrect and meaningless access control policies opening up a backdoor in the computer system to attackers. Even though this problem persisted in every identified NLP-based policy generation pipeline, non of the extracted literature attempted to solve it. One viable solution would be to adapt the human-in-the-loop concept to involve a human administrator in policy generation to validate the model-generated policies and provide feedback to improve the ML/NLP model further. In human-in-the-loop machine learning, researchers mainly identified 3 main types of interactions between machine learning and human that can help the learner (ML model) to improve using human expertise such as Active Learning (AL), Interactive Machine Learning (IML) and Machine Teaching (MT) \cite{mosqueira2023human}. Among the above 3 types, AL is a promising technique for policy generation, in which the learner (i.e. ML/NLP model) requests an oracle (i.e. the administrator) to label selected examples, or provide additional information iteratively that are relevant to the learning process \cite{mosqueira2023human}. By adopting the AL technique, the administrator is participating in the policy generation process by providing feedback based on the model outputs (i.e. generated machine-executable policies) to ensure their reliability and completeness while allowing the model to be retrained with corrected labels via scheduled online training. Therefore, \textbf{adapting human-in-the-loop techniques in policy generation} to increase the completeness and correctness of the generated access control policies can be addressed in future research. Furthermore, as we reported in Section \ref{subsubsec:limit_nlp} and discussed in Section \ref{sec:discussion}, \textbf{developing an annotated policy generation dataset} will complement future research and will make it possible to adapt LMs and LLMs extensively in future. 


% As a result, administrators might feel overwhelmed and stressed due to this repetitive nature of the manual policy generation \cite{palmer_2021}.


% When it comes to administrators, access control configuration failures can happen due to 2 main reasons. First is the lack of experience of the administrator \cite{reeder2011more, maxion2005improving}. If the administrator does not have experience in using access control models and languages, often they fail to generate correct access control policies causing access control failures \cite{inglesant2008expressions, stepien2009non}. For example, in 2004, one political party on the United States Judiciary Committee gained access to the confidential memos of the opposing party, stored in a shared server causing the "Meomogate Scandal" \cite{maxion2005improving, reeder2008expandable}. Interestingly, the administrator they hired to protect the memos from unauthorized access, was a fresh college graduate who did not have system administration experience. To avoid such scenarios, previous literature proposed GUI-based policy authoring and visualization tools \cite{shi2011controlled, inglesant2008expressions, stepien2009non, bertard2020using, turner2017proposed, brostoff2005r, zurko1999user, karat2006evaluating, johnson2010usable, johnson2010optimizing, maxion2005improving, cao2006intentional, reeder2007usability, reeder2008expandable, morisset2018visabac, brodie2005usable, brodie2006empirical}. Those tools were developed to guide administrators to produce access control policies manually without focusing on the technicalities of the access control models or languages \cite{shi2011controlled}. However, manual policy generation is a repetitive, laborious, and error-prone task \cite{narouei2017identification, nobi2022machine}. The administrator has to carefully generate and configure policies so that the proper access were provided to correct resources repetitively \cite{reeder2008expandable, reeder2011more, maxion2005improving}. As a result, administrators might feel overwhelmed and stressed due to this repetitive nature of the manual policy generation \cite{palmer_2021}, regardless of their expertise. 
% Consequently, those mental conditions will affect the administrators' critical decision-making ability, causing accidental human errors \cite{palmer_2021}.

21.6\% of the extracted publications propose text editors to provide guidance to the system administrators to write access control policies \cite{stepien2009non, stepien2014non, zurko1999user, brodie2005usable, brodie2006empirical, brostoff2005r, reeder2007usability, vaniea2008evaluating, inglesant2008expressions, shi2011controlled, karat2006evaluating}.


Properly formatted high-quality access control policies often increase the manageability of the policy configuration system \cite{bertino2018challenge}. For example, when there are multiple policy authors involved in policy configuration, having policies with consistent format helps to understand policies written by each other, and will help solving conflicts between those policies \cite{bauer2009real}. Therefore, in order to guide policy authors (i.e. system administrator) to write properly formatted policies according to pre-defined policy structures, template-based policy authoring interfaces were introduced \cite{johnson2010optimizing, johnson2010usable, rosa2020parser, turner2017proposed}. 

Nevertheless, manually generating policies using GUIs and automated policy generation using NLP techniques both introduce their unique but complementary challenges for the policy generation process \cite{kaur2021human}. For instance, manual policy authoring causes overhead due to the lack of automation, while automated policy generation often fails to generate correct policies due to the lack of human supervision. Therefore, we have to identify the trade-off between manual (i.e., GUI-based) and automated (i.e., NLP-based) policy generation approaches to develop more effective policy generation tools. Identifying that trade-off will allow us to develop better policy generation tools with \textbf{improved usability and reliability} while \textbf{reducing the administrator's overhead}. As a result, human errors due to the administrator's overhead, as well as algorithmic errors due to inaccurate policy generation pipelines, can be reduced. 
% combine the usability of graphical policy authoring and visualization tools with the reliability of automated policy generation to develop future frameworks. 
% As a result, administrators will be able to participate in the policy generation process via a usable GUI in a way that their overhead is minimized and the reliability of automated policy generation is increased. 
Therefore, to identify that trade-off, first, we need to identify both the existing graphical policy authoring and visualization tools, the NLP-based automated policy generation frameworks, and their limitations. However, so far, there are no systematic literature reviews that evaluate both the above approaches and point out their limitations. Therefore, this research focuses on conducting a SLR to answer two key research questions, RQ1 and RQ2.


\section{Results}

Access control failures due to policy configuration mistakes by system administrators can result in drastic data breaches putting an entire organization at risk of financial and reputation damage \cite{Heiligenstein_2023, bauer2009real}. Therefore in order to avoid such access control failures, previous research has proposed numerous tools and frameworks that are designed to help the administrator correctly generate as well as visualize access control policies. However, those tools and frameworks are not usable or reliable enough to help the administrator generate accurate access control policies with less overhead. This raises two main questions: What are those tools and frameworks? and what their limitations are. To answer those questions, we conducted the thematic analysis \cite{cruzes2011recommended}, which led us to identify two main approaches taken by previous literature to develop such tools and frameworks as shown in Fig. \ref{fig:tools}. They are \textbf{a) graphical policy authoring and visualization} \cite{stepien2014non, brostoff2005r, zurko1999user, vaniea2008access, johnson2010optimizing, maxion2005improving, cao2006intentional, reeder2007usability, reeder2008expandable, morisset2018visabac,stepien2009non, reeder2011more, morisset2018building, bertard2020using, rosa2020parser, turner2017proposed}, and \textbf{b) NLP-based automated policy generation} \cite{fatema2016semi,xiao2012automated,slankas2012classifying,ye2016identify,slankas2013implementing,fornara2016modeling,perry2013modular,slankas2014relation,jones2015towards,tanoli2018towards,amato2013semantic,slankas2013access,slankas2013accessid,rosa2020parser,brodie2006empirical,alohaly2016better,vaniea2008evaluating,karat2006evaluating,inglesant2008expressions,basile2010ontology,turner2017proposed,reeder2007usability,brodie2005usable,das2018hype,shen2021using,xia2022automated}.

 Tools used for graphical policy authoring and visualization often provide a usable interface that allows system administrators to write and visualize policies manually \cite{stepien2009non, morisset2018building, reeder2007usability}. Previous literature proposed graphical user interfaces (GUIs) specifically designed for policy authoring, such as text editor-based \cite{brostoff2005r, zurko1999user, stepien2009non, stepien2014non} and template-based authoring tools \cite{johnson2010optimizing, johnson2010usable, rosa2020parser, turner2017proposed}, tools designed for policy visualization, such as graph-based visualization tools \cite{morisset2018building, morisset2018visabac, bertard2020using}, and tools that facilitate both policy authoring and visualization at the same time, such as access matrix-based policy authoring and visualization tools \cite{reeder2008expandable, reeder2011more, vaniea2008access, cao2006intentional, maxion2005improving, vaniea2008evaluating}. Text editor-based tools guide the administrator to build a policy by separately defining its policy components using text boxes \cite{stepien2009non, stepien2014non} or combo boxes \cite{brostoff2005r} as shown in Fig. \ref{fig:gui_tools}(a). On the other hand, as shown in Fig. \ref{fig:gui_tools}(d), template-based tools provide one \cite{turner2017proposed, rosa2020parser} or more pre-defined templates \cite{johnson2010usable, johnson2010optimizing} to write the policy according to a standard format while preserving the semantic meaning of the intended policy. However, neither of those types of tools visualizes the already written policies and their rules graphically as a single diagram. Therefore, the important contextual information from all the policies, which is essential especially when resolving conflicts between policies, will not be available to the administrator \cite{reeder2008expandable, bauer2009real}, leading to mistakes when authoring policies. With that in mind, access matrix-based tools that allow the administrator to write (i.e., policy authoring) as well as visualize (i.e., policy visualization) all the policies in a single matrix (representing users as rows and resources as columns) were developed \cite{reeder2008expandable, reeder2007usability, maxion2005improving}.  However, the access matrices can be hard to navigate if the number of users and resources is high in the organization \cite{morisset2018building}. For example, Reeder et al., \cite{reeder2008expandable}, developed an ``Expandable grid" for Microsoft Windows XP Operating System (Fig. \ref{fig:gui_tools}(b)) for visualizing and authoring computer security policies. The administrator then has to scroll through rows and columns to find the intersection to provide permission if the number of rows (i.e., users) or columns (i.e., resources) is high. When doing that, sometimes the administrator will mistakenly provide the incorrect user access to an incorrect resource, causing access control failures (off by one error \cite{reeder2008expandable}). As a solution, graph-based visualization tools (Fig. \ref{fig:gui_tools}(e)) were proposed to effectively represent the high number of users and resources in the organization \cite{morisset2018visabac}. Overall, these tools provide a higher level of abstraction, allowing administrators to focus on the high-level access control requirements of the organization rather than low-level technical details of the access control model, language, or syntax \cite{stepien2009non}. 
 % Therefore, many studies have shown that these tools improve efficiency, and accuracy while reducing the cognitive load in policy configuration \cite{reeder2008expandable, reeder2011more, karat2006evaluating, maxion2005improving, stepien2009non, stepien2014non}. 
 However, the proposed graphical tools have their own limitations. As the previous research revealed, some of the graphical policy authoring tools lack the flexibility \cite{brodie2006empirical, brodie2005usable, karat2006evaluating, vaniea2008access, turner2017proposed, rosa2020parser, shi2011controlled, inglesant2008expressions} and do not support complex access control policies \cite{stepien2009non, stepien2014non, bertard2020using, morisset2018building, morisset2018visabac, reeder2008expandable, reeder2011more, maxion2005improving, cao2006intentional}, preventing the administrator to build custom and complex policies with different access requirements. Furthermore, the graphical representation of the policies as well as the GUI features of the tools, often are subjected to inconsistent interpretations by the administrators \cite{brostoff2005r, morisset2018building, morisset2018visabac}.  Because administrators are often not security experts and come from non-technical backgrounds without much system administration experience \cite{brostoff2005r, reeder2007usability, jaferian2014authorize}. Therefore, these limitations make the existing graphical policy authoring and visualization tools less usable for accurate policy configuration (e.g., Setting up file permissions in Operating systems).

On the other hand, graphical policy authoring and visualization is a manual, repetitive, and laborious process \cite{narouei2015automatic}. Therefore, IT security professionals consider this process an overhead \cite{botta2007towards}, which can cause fatigue and stress impairing their critical decision-making ability \cite{palmer_2021}. As a solution, NLP-based automated policy generation frameworks were introduced that utilize ML and NLP techniques to generate machine-executable access control policies from documents that contain high-level access control requirement specifications written in natural language \cite{narouei2015towards}, with almost no human involvement. Those proposed automated policy generation frameworks usually consist of 4 main steps. First, the natural language (NL) documents were pre-processed by using techniques such as sentence tokenization \cite{slankas2012classifying, slankas2013access, slankas2013accessid, slankas2014relation, narouei2015automatic, narouei2015towards, narouei2017identification, narouei2017towards, narouei2018automatic, tanoli2018towards, xiao2012automated}, word tokenization \cite{narouei2015automatic, narouei2015towards, narouei2017identification, narouei2017towards, narouei2018automatic, alohaly2018deep, alohaly2019automated, alohaly2019towards, tanoli2018towards, heaps2021access, yang2021purext, singru2020efficient, amato2013semantic}, filtering unwanted sections in the document \cite{slankas2012classifying, slankas2013access, narouei2017identification, narouei2017towards}, stop word removal \cite{tanoli2018towards, singru2020efficient} etc. Secondly, the natural language access control policies (NLACPs) were identified using text classification techniques such as Support Vector Machines (SVM) \cite{slankas2013access, slankas2013accessid}, k-Nearest Neighbours \cite{slankas2014relation, slankas2012classifying, slankas2013access, slankas2013accessid, narouei2015automatic, narouei2018automatic, narouei2015towards}, Transformers \cite{heaps2021access, xia2022automated}, Naive Bayes \cite{slankas2013access, narouei2017identification} etc. Once the NLACPs were identified, machine-executable policies should be built from the NLACPs. Therefore, as the third step, necessary policy components (i.e. subjects, actions, resources, etc.) were extracted by employing information extraction techniques including syntactic parsing \cite{brodie2006empirical, xiao2012automated, vaniea2008evaluating, karat2006evaluating, reeder2007usability, brodie2005usable, slankas2013access, narouei2017identification, ye2016identify, yang2021purext, slankas2014relation, alohaly2019towards, tanoli2018towards, xia2022automated, shi2011controlled, fatema2016semi, inglesant2008expressions, turner2017proposed, shen2021using, basile2010ontology, alohaly2018deep, alohaly2019automated}, semantic role labeling (SRL) \cite{xia2022automated, narouei2015automatic, narouei2018automatic, yang2021purext, narouei2017towards, narouei2015towards}, named entity recognition (NER) \cite{heaps2021access, zhu2021unstructured} or a combination of multiple extraction techniques (e.g. SRL and dependency parsing were used together to extract component in a more granular way \cite{xia2022automated, narouei2015automatic, yang2021purext, narouei2015towards, alohaly2019towards}). Finally, the extracted policy components were transformed into a policy language such as XACML (eXtensible Access Control Markup Language) \cite{xia2022automated, turner2017proposed, amato2013semantic, slankas2012classifying, fatema2016semi, brodie2005usable, vaniea2008evaluating, shi2011controlled, karat2006evaluating, brodie2006empirical}, PERMIS (Policy Enforcement through Role-based access control Mechanisms Implementation and Specification) \cite{inglesant2008expressions, shi2011controlled}, EPAL (Enterprise Privacy Authorization Language) \cite{brodie2006empirical, brodie2005usable, karat2006evaluating, vaniea2008evaluating} or into an intermediate representation such as an ontology \cite{shi2011controlled, inglesant2008expressions, fornara2016modeling, tanoli2018towards, basile2010ontology}. 
% Finally, the generated policies were evaluated either by using the F1-score \cite{xiao2012automated, xia2022automated, slankas2013access, slankas2013accessid, slankas2012classifying, slankas2014relation, narouei2015towards, narouei2017towards, narouei2018automatic, narouei2017identification, alohaly2018deep, alohaly2019automated, alohaly2019towards, heaps2021access, brodie2006empirical, shen2021using, yang2021purext, zhu2021unstructured} or the accuracy \cite{singru2020efficient} in the extracted literature. 
Since human involvement is minimum in the above steps, the room for human errors is minimum. On the one hand, the policy generation process will be more efficient than the manual policy generation since the entire process is done by an algorithm \cite{xiao2012automated, xia2022automated, slankas2014relation, slankas2013access, narouei2015automatic, alohaly2018deep}.

Despite helping the administrator by automating the policy generation, we identified several limitations of existing policy generation frameworks \cite{slankas2014relation, xiao2012automated, xia2022automated, heaps2021access, alohaly2016better, alohaly2018deep, alohaly2019automated, narouei2015automatic, narouei2015towards, narouei2017identification, brodie2005usable, brodie2006empirical, karat2006evaluating, vaniea2008evaluating}. Our SLR findings revealed that the lack of domain-related high-quality datasets hinders the development of more accurate frameworks to automate access control policy generation \cite{nobi2022machine, xia2022automated} as it prevents the researchers from properly fine-tuning the ML/NLP models to make the general purpose model to adapt in the access control domain. Also, consequently, it makes the existing automated policy generation frameworks not reliable enough to operate without human supervision \cite{del2022systematic, xia2022automated, narouei2015automatic} since the policy generation framework is not properly adopted to the access control domain. Furthermore, some of the existing frameworks, especially the ones that use rule-based information extraction techniques \cite{xiao2012automated, brodie2006empirical}, cannot handle ambiguities in NLACPs. Because they expect clear and complete NLACPs written according to pre-defined sentence structures that can be parsed using their grammar rules, \cite{brodie2006empirical}. If the NLACP is ambiguous and consequently not agreeing with parsing rules, rule-based parsers fail to identify policy components, resulting in incomplete or missing access control policies. Therefore, to avoid such scenarios, previous literature decided to use a controlled natural language (CNL) that forces administrators to write policies according to pre-defined syntax or templates, restricting the allowed vocabulary and grammar \cite{brodie2006empirical, inglesant2008expressions, shi2011controlled}. However, this restriction limits the flexibility of policy authoring, making it difficult for administrators to transfer their intended policies to the authorization system \cite{inglesant2008expressions}. 

In summary, even though graphical policy authoring and visualization tools guide the administrator to write policies, the \textbf{overhead} due to the manual policy authoring and their own limitations induce human errors, making them \textbf{less usable} for effective policy authoring and visualization. 
% On the one hand, the manual and repetitive graphical policy authoring techniques significantly contribute to the overhead of administrators due to the lack of automation. 
On the other hand, even though the existing automated policy generation frameworks reduce that overhead significantly, they are \textbf{not reliable enough} to use without human supervision. Because those frameworks might not generate policies accurately every time (i.e., automation surprise \cite{kaur2021human}) as they are often not properly trained to handle complex and ambiguous policies. Therefore, to develop a better and more effective tool, it is crucial to improve the usability and reliability (i.e., usability-security trade-off) of the above two policy generation approaches (i.e., graphical policy authoring and visualization and NLP-based automated policy generation) together while reducing the administrator's overhead. To do that, first, we have to deep dive into the existing graphical policy authoring and visualization tools, as well as NLP-based automated policy generation frameworks, to understand how they work and where the limitations are. 
With that motivation, 
% to develop a more effective tool, it is important to identify how the existing graphical policy authoring and visualization tools and NLP-based automated policy generation frameworks can be further improved and how to combine them in a way that they complement each other. With that in mind, 
in the next two subsections, we discuss graphical policy authoring and visualization tools, NLP-based automated policy generation frameworks, and their limitations in detail. A summary of the results can be found at \url{https://cutt.ly/uwdS3ACt}.


Therefore, we suggest to improve the reliability of automated policy generation frameworks in four ways. First, we can utilize a superior NLP model, which is proven to be effective in text classification \cite{xia2022automated} and information extraction \cite{shi2019simple} while handling ambiguities and complexities of natural language sentences. In that case, we can consider transformer-based language models as one alternative \cite{vaswani2017attention} as they were pre-trained using a massive amount of data \cite{brown2020language, raffel2020exploring}, enriching them with knowledge on nuances of ambiguous and complex English sentences. However, if we utilize a general-purpose NLP model such as a model trained to predict the next token \cite{brown2020language}, or a model trained to find a masked word in a sentence \cite{devlin2018bert} to generate access control policies without adapting it to access control policy identification and component extraction, we may not able to achieve good results as they are not familiar with nuances of access control policy generation specifically \cite{weiss2016survey, alohaly2019automated}. Therefore, we suggest using transfer learning and fine-tuning techniques, which we revealed are rarely used in the policy generation domain, to adopt a general-purpose NLP model to identify NLACPs and extract their components accurately. However, to fine-tune a NLP model properly, we need to have a proper domain-related dataset, which is lacking in access control policy engineering domain \cite{narouei2017identification, xia2022automated}. Therefore, we encourage the research community to develop such datasets by pointing out some of the important qualities that a proper dataset should have as the next way of improving the reliability of the automated policy generation framework. Even if we properly fine-tuned a NLP model to identify NLACPs and extract their components, those models often do not produce the expected result every time \cite{kaur2021human}. If those unexpected results (i.e., identified policies or extracted policy components) were used to build machine-executable policies, those policies would often be incorrect or incomplete, leading to access control failures. Therefore, to avoid such situations as much as possible, we suggest utilizing the administrator's expertise as a way of providing feedback on model-generated outputs by adding the human administrator into the policy generation pipeline.

\begin{itemize}
    \item \emph{\textbf{Utilizing transformer-based language models (LMs)}} - With the invention of the Transformer \cite{vaswani2017attention}, NLP domain has massively expanded after 2017. NLP researchers used this transformer architecture based on an encoder and a decoder to develop LMs such as Encoder-only LMs (e.g., BERT \cite{devlin2018bert}), decoder-only LMs (e.g., GPT-2 \cite{brown2020language}) and encoder-decoder LMs (e.g., T5 \cite{raffel2020exploring}). Later, by further adding trainable parameters to LMs, Large Language Models (LLMs) were introduced (e.g., GPT-4 \cite{openai2023gpt4}). These LMs and LLMs were pre-trained on gigabytes of data enriching them with a significant understanding of NL. Thus, upon carefully fine-tuning, they were used to produce state-of-the-art results in various NLP tasks such as SRL \cite{shi2019simple}. Therefore, utilizing transformer-based LMs and LLMs would be a promising approach for reliable access control policy generation while handling the ambiguities of unconstrained natural language \cite{heaps2021access, xia2022automated}. However, only 2 of the extracted publications attempted to employ transformers for access control policy generation. Furthermore, none of the extracted articles attempt to generate access control policies directly from NLACPs without extracting components and transforming them separately. It may remove many post-processing and decision-making tasks such as predicate pruning \cite{xia2022automated} and avoids using multiple LMs sequentially to carry out sub-tasks in policy generation such as ACP classification, access type classification, etc. \cite{heaps2021access}. Consequently, it will increase the efficiency and flexibility of policy generation. 
    % Therefore, the feasibility of generating machine-executable policies directly from NLACPs using decoder-only or encoder-decoder language models can be explored in future research.

    \item \emph{\textbf{Fine-tuning and Transfer learning}} - Language models (LMs) cannot be used directly to identify policies or extract their components. Because they were trained using a general pre-training objective such as Masked Language Modeling \cite{devlin2018bert} or Next token prediction \cite{radford2019language}. Therefore, to adapt them to the access control domain, those LMs should be fine-tuned using a domain-related dataset (such as the one shown in Table \ref{tab: dataset}). However, in fine-tuning, all the trainable parameters of the LM will be updated in the training process. Therefore, a significant amount of data is required to achieve good results. On the other hand, "Transfer learning" is the process of improving a ML/NLP model pre-trained in a different domain by transferring information from a related domain \cite{weiss2016survey}. This technique allows a ML model to be trained with fewer data points in contrast to fine-tuning, related to a specific task, and improves its accuracy in the task. For example, consider access policy component extraction. Even though there are no specifically trained NLP models to extract policy components, transfer learning can be used to train a NLP model pre-trained on a related information extraction task (e.g., semantic parsing or semantic role labeling) using a domain-related dataset. This helps the ML/NLP model to achieve a high accuracy quickly compared to training the model from scratch. This technique was successfully applied on a few occasions among the extracted literature \cite{heaps2021access, xia2022automated, narouei2018automatic, zhu2021unstructured} and proved that it would increase the accuracy of policy generation \cite{narouei2015automatic}. Even though fine-tuning and transfer learning are effective techniques to adopt relatively small NLP models to access control policy generation, they might become infeasible when it comes to LLMs, which contain billions of parameters. Therefore, adapting them to the access control domain will not only require a larger dataset but also it will need more computing resources. As a solution, Parameter Efficient Fine Tuning (PEFT) \cite{houlsby2019parameter} can be utilized, which adds a small number of trainable parameters to the LLM and only fine-tunes them by freezing the parameters of the original LLM. 

    \item \emph{\textbf{Developing a high-quality dataset}} - As we reported in Section \ref{subsubsec: nlpgen}, many extracted studies have raised concerns on the scarcity of a proper NLACP dataset \cite{narouei2017towards, narouei2018automatic, narouei2017identification, alohaly2019automated, xia2022automated, yang2021purext}. Therefore, developing an annotated dataset would significantly contribute to future research in the access control policy generation domain. With that motivation, we suggest the following qualities a proper dataset should have to support improving the reliability of NLP-based frameworks. 
    \begin{itemize}
        \item \emph{High-quality} - The dataset should contain high-quality data with accurate and consistent labeling, minimal noise, and bias. This ensures that the resulting model is accurate and reliable.
    
        \item \emph{Trustworthy} - The dataset should be created by following the common principles such as FAIR (Findable, Accessible, Interoperable, Reusable) principles \cite{wilkinson2016fair}. To ensure the quality of the data, multiple domain experts should be involved in annotating the data. Finally, the inter-coder agreement should be calculated using a metric such as Cohen Kappa \cite{mchugh2012interrater}. Ideally, the kappa value ($\kappa$) should be greater than or equal to 0.61 ($\kappa$ $\geq$ 0.61) for a substantial agreement \cite{mchugh2012interrater}.  
    
        \item \emph{Diverse} - The dataset should contain NLACPs with a wide range of semantic and syntactic structures. This helps ensure that the resulting model is robust and generalizes well to new data.
    
        % \item \emph{Sufficient} - The dataset should be large enough to sufficiently represent different access control policy structures but not so large enough that it becomes difficult to handle. This ensures the model is properly trained and will not "overfit" or "underfit" the training data. 
    
        \item \emph{Accessible} - The dataset should be publicly available to make it easily accessible to researchers. This ensures that the experiments can be replicated and can be used as a baseline for future work.
        
    \item \emph{\textbf{Adapting human-in-the-loop concept to improve the reliability of policy generation}} - By looking at the developed NLP-based access control policy generation techniques, it is evident that a ML/NLP model alone itself cannot reliably generate machine-executable access control policies without the administrator's supervision \cite{xia2022automated, heaps2021access, narouei2018automatic, narouei2017towards, narouei2015automatic}. 
    % Especially when the models trained on insufficient and less-quality datasets with low accuracy values are involved \cite{xia2022automated, heaps2021access, narouei2018automatic, narouei2017towards, narouei2015automatic}. 
    For instance, Heaps et al. reported that their BERT-based policy component extraction model falsely identified "admitted" as a user, as it is close to the word "administrator" \cite{heaps2021access}. If such false positives were \textbf{applied blindly without correcting them}, they could result in incorrect and meaningless access control policies opening up a backdoor in the computer system to attackers. Even though this problem persisted in every identified NLP-based policy generation pipeline, none of the extracted literature attempted to solve it \cite{xia2022automated, heaps2021access, narouei2015automatic, alohaly2019automated}. Therefore, one viable solution would be to adapt the human-in-the-loop concept to involve a human administrator in policy generation to validate the model-generated policies and provide feedback to refine the ML/NLP model output further \cite{mosqueira2023human}. However, we should not expect the administrator to be involved in policy generation every time a model generates a policy, as it would increase the administrator's overhead. Therefore, to identify when to involve the administrator in policy generation, the policy generation frameworks should be designed to provide adequate and usable feedback to the administrator, clearly pointing out the occasions that are more likely for the model to make mistakes (e.g., occasions where the policy components were identified with low confidence), so that the administrator can join the policy generation only in that situations. In this way, administrator will not always interacting with automated policy generation.

    
\end{itemize}
\end{itemize}



However, ML/NLP models can also make mistakes, as they are not 100\% accurate. For instance, NLACPs are often abstract and ambiguous \cite{narouei2017identification}. If the information extraction technique is \textbf{not robust and cannot handle ambiguities}, it will fail to identify all the necessary policy components, resulting in incomplete access control policies. Therefore, to avoid such ambiguities, CNL was used to write NLACPs, which forces administrators to use non-natural grammar to write their policy requirements in high-level requirement specification documents, \textbf{reducing the flexibility} of policy authoring, consequently reducing the flexibility of the policy generation. Also, if the information extraction technique's \textbf{accuracy is not enough}, it tends not to identify or incorrectly identify policy components, also resulting in incorrect access control policies \cite{heaps2021access}. If those incorrect policies are applied to an authorization system without being verified by the system administrator, they will cause access control failures, leading to data breaches. However, the reliability can be improved by using a sufficient and properly annotated dataset to train the information extraction model. Even though developing a properly annotated dataset is laborious and time-consuming, we consider it worthwhile since it reduces the chance of generating incorrect access control policies by the policy generation frameworks, reducing the probability of access control failures due to algorithmic errors. Unfortunately, the problem remains open and unsolved due to the \textbf{lack of domain-related datasets}. 



% What are the fundamental reasons behind such data breaches? and Who is responsible? 

% In April 2021, the confidential information of over 533 million Facebook users was publicly posted in an online hacking forum \cite{Holmes_2021}. The leaked data appeared to have been scraped in 2019 when a group of hackers exploited a vulnerability in Facebook's contact importer, which was used to find people online by entering phone numbers \cite{Heiligenstein_2023}. However, Facebook decided against notifying the 533 million users whose confidential information had been leaked. As a result, in November 2022, Meta (formerly known as Facebook) had to pay €265 million to Ireland Data Protection Commission for violating the European Union’s General Data Protection Regulation (GDPR) as part of this incident \cite{Heiligenstein_2023}. These kinds of data breaches raise 2 basic questions: What are the fundamental reasons behind such data breaches? and Who is responsible? 



Graphical policy authoring can be done using text-editor \cite{brostoff2005r, zurko1999user, stepien2009non, stepien2014non} or template \cite{johnson2010optimizing, johnson2010usable, rosa2020parser, turner2017proposed} based policy authoring tools that guide the system administrators to write access control policies manually with the help of an interactive graphical user interface. However, they do not provide ways to visualize access control policies, making it difficult for administrators to understand and interpret the existing policies with a low cognitive load \cite{vaniea2008access}. Therefore, as solutions, access matrix-based tools \cite{reeder2008expandable, reeder2011more, vaniea2008access, cao2006intentional, maxion2005improving, vaniea2008evaluating} that allow the administrator to write and visualize access control policies, and graph-based policy visualization tools \cite{morisset2018building, morisset2018visabac, bertard2020using} that visualize policies in terms of graphs/trees were introduced. Nevertheless, all the above tools are designed to facilitate manual and repetitive policy configuration \cite{narouei2017identification}. Therefore, those tools increase the overhead of the system administrator, causing fatigue and stress, impairing their critical decision-making ability \cite{palmer_2021}. As a solution, NLP-based automated policy generation frameworks were then introduced that utilize ML and NLP techniques to generate machine-executable access control policies from documents that contain high-level requirement specifications written in natural language \cite{shi2011controlled, alohaly2018deep, alohaly2021hybrid, amato2013semantic, fatema2016semi, slankas2013access, heaps2021access, slankas2013accessid, brodie2006empirical, xia2022automated, alohaly2019automated, xiao2012automated, narouei2018automatic, narouei2015automatic, slankas2012classifying, singru2020efficient, vaniea2008evaluating, karat2006evaluating, inglesant2008expressions, liu2017automated, narouei2017identification, ye2016identify, slankas2013implementing, perry2013modular, basile2010ontology, yang2021purext, slankas2014relation, narouei2017towards, alohaly2019towards, narouei2015towards, tanoli2018towards, zhu2021unstructured, brodie2005usable, shen2021using, abdelgawad2023synthesizing}, with almost no human involvement. Therefore, the administrator's overhead can be reduced, and, in turn, accidental human mistakes in access control policy configuration will also be reduced. 

However, as we identified, graphical policy authoring and visualization tools are often prone to human errors, making them less usable for preventing access control failures \cite{reeder2007usability, reeder2008expandable, reeder2011more, maxion2005improving, johnson2010usable}. 
% However, as we identified, the usability and reliability issues of the aforementioned tools and frameworks make them ineffective in secure access control policy configuration. For instance, the proposed graphical policy authoring and visualization tools are often not flexible enough to support the unique and complex access requirements of an organization with , while policy visualization techniques are often subject to misinterpretations due to their lack of explainability \cite{maxion2005improving}. 
On the other hand, ML/NLP techniques used to develop existing automated policy generation frameworks were not properly adapted to the access control domain, making them unreliable to use without human supervision \cite{kaur2021human, xia2022automated, heaps2021access}. Therefore, to avoid access control failures, it is essential to improve usability and security in terms of reliability (i.e., address usability-security trade-off) in graphical policy authoring and visualization tools and NLP-based automated policy generation frameworks. 
% By doing so, it will be possible to develop secure policy generation frameworks that utilize the reliability and efficiency of automated policy generation together with a usable policy configuration interface for the system administrators to productively interact with the policy generation process. 
To do that, we have to dive deep into those tools and frameworks to understand how they work and where their limitations are. Identifying those limitations will help identify ways to improve the usability and reliability of access control policy generation and, in turn, help develop more effective policy generation frameworks that are usable and reliable for avoiding access control failure. Therefore, in the next two subsections, we discuss graphical policy authoring and visualization tools, NLP-based automated policy generation frameworks, and their limitations in detail. 




\section{Conclusion 1}
Nevertheless, we would like to point out three limitations of those studies that proposed graphical tools that can be addressed in future research apart from the proposed usability improvements Section \ref{subsec: discuss_gui}. (1) As we found out, the existing studies that propose such graphical tools did not often evaluate their usability in terms of the mentioned usability components \cite{stepien2009non, stepien2014non, turner2017proposed, rosa2020parser}. For example, none of the extracted studies have conducted long-term studies to measure the memorability \cite{saket2016beyond} of the proposed policy authoring and visualization interfaces. These would help improve the interface so that the administrator can easily adapt to the interface even after not using the interface for some time \cite{nielsen1994usability}. (2) As we discussed, providing adequate feedback is one technique to reduce errors in policy configuration \cite{xu2017system}. However, not only almost all the graphical tools we examined do not provide feedback or error messages pointing out the error, its location, solutions, and its severity, but also none of those studies have focused on designing those messages in a way that they are easily understandable to system administrators, via user studies. (3) When evaluating those graphical tools, previous literature did not often use proper evaluation questionnaires such as PSSUQ \cite{fruhling2005assessing}, which consists of 19 items aimed to address five system usability characteristics: quick completion of work, ease of learning, high-quality documentation and online information, functional adequacy and rapid acquisition of usability experts and several different user groups, or System Usability Scale (SUS) \cite{brooke1996sus}, a Likert scale containing ten items that can be used to evaluate the usability of access control policy configuration tools. If we take a closer look at the questions of those questionnaires, we can see that they focus on identifying whether Nielsen's five usability components were addressed in user interfaces or not. Therefore, by utilizing those questionnaires, we can ensure that the developed policy configuration tool is learnable, efficient, and memorable, reducing errors and improving subjective satisfaction.
% because most of them do not support complex access control policies, are not flexible, and are prone to inconsistent interpretations. 
% Furthermore, graphical policy authoring and visualization is a manual, repetitive, and laborious process, which is considered an overhead that makes the administrators stressed and fatigued. 

On the other hand, NLP-based automated policy generation frameworks were then developed that generate machine-executable policies from NLACPs automatically by removing the administrator considerably from the policy generation. However, as we found out, the policy generation frameworks are not reliable enough to use without human supervision, as most of those existing pipelines cannot handle complex and ambiguous NLACPs accurately. However, as we found out, almost all the automated policy generation frameworks did not empirically evaluate how those frameworks help administrators to effectively generate policies with less overhead. Such empirical evidence will be important to evaluate their reliability in real-world scenarios. In order to improve reliability, as we discussed, the LMs should be trained properly using domain-related datasets \cite{xia2022automated}. However, as we highlighted, the access control policy generation domain is suffering from a lack of domain-related datasets \cite{xia2022automated, slankas2014relation}. Therefore, as future works, we encourage researchers to develop such datasets with accurate annotations and make them publicly available to help develop more reliable access control policy generation frameworks in the future. 
% Finally, even if more reliable automated policy generation frameworks are developed in the future, they might not be accurate every time, as . Those occasions result in incorrect access control policies that might lead to data breaches. Therefore, as a solution, we suggest utilizing the human-in-the-loop technique \cite{wu2022survey} in a productive way to utilize the administrator's expertise to refine the incorrect model outputs when necessary.
% Furthermore, the lack of domain-related datasets has prevented those NLP frameworks from training properly, making them even less accurate to operate without human supervision.





\section{Conclusion 2}

This systematic literature review presents a comprehensive overview of the tools and frameworks proposed for access control policy generation by the system administrator. Our review identified two main approaches that were followed by previous literature to develop those tools and frameworks: (a.) graphical policy authoring and visualization and (b.) NLP-based automated policy generation. Tools designed for graphical policy authoring and visualization provide more intuitive platforms that guide administrators to write and visualize access control policies even without having knowledge about access control models, languages, and syntax. However, our review revealed that the existing graphical policy authoring and visualization tools not only increase the administrator's overhead but also suffer from a lack of usability, inducing accidental human errors. 
% Therefore, to avoid such errors, we provided guidelines on how to improve the usability of those tools in terms of their learnability, memorability, and subjective satisfaction while reducing the errors and improving the efficiency by referring to Nielsen's usability components \cite{nielsen1994usability}.
On the other hand, NLP-based automated policy generation frameworks were then developed that generate machine-executable policies from NLACPs automatically by removing the administrator considerably from the policy generation. However, as we found out, the policy generation frameworks are not reliable enough to use without human supervision, as most of those existing pipelines cannot handle complex and ambiguous NLACPs accurately. Therefore, based on our findings, we have provided several design guidelines that would help improve the usability of policy authoring and visualization tools according to Nielsen's usability components \cite{nielsen1994usability}: learnability, memorability, efficiency, errors, and subjective satisfaction, as well as improve the reliability of automated policy generation frameworks by selecting best techniques for pre-processing, text classification, information extraction, and information transformation. 

Therefore, based on the above results of the review, we came to 3 conclusions that would drive future research. First, the existing graphical policy authoring and visualization tools should be further improved to make them more usable for system administrators. By doing so, the probability of accidental human errors in policy configuration can be reduced. Secondly, the NLP-based automated policy generation frameworks should also be improved by utilizing more reliable NLP techniques trained on a high-quality annotated dataset to make the policy generation more reliable. These improvements will help to reduce the policy generation overhead of the system administrator while preserving accuracy and efficiency. 
% However, as we found out, utilizing completely manual or completely automated tools in policy generation is not effective, no matter how usable or reliable they are. 
Therefore, finally, we suggest the development of policy generation frameworks that use a more reliable policy generation pipeline together with a usable interface to utilize the administrator's expertise productively. By doing so, we will be able to generate secure access control policies in a usable and efficient way. 

\section{Intro}

% These kinds of access control failures can happen due to mistakes by either end-users, software developers, or system administrators \cite{inglesant2008expressions} in different severities. For example, when it comes to social networks such as Facebook, end users control access to their private photos and personal information. Poorly configured privacy settings of their Facebook profile could result in unintended exposure of personal data to a broader range of audiences \cite{digioia2005social, smetters2009users}. While this can have serious privacy implications, such as identity theft \cite{Picchi_2018}, the scope of impact is generally limited to the user's own account and their connections within the social media platform. Next, software developers implement access control in their developed applications to provide a secure user experience to their users \cite{li2019evaluation, zhu2015mitigating}. If developers do not correctly implement access control in one of those applications, the negative impact is typically limited to the application itself and the users of that application. For example, if developers do not properly implement access control in an application such as a file management application, anyone might be able to access and steal anyone's files, affecting the data it stores and the owner of the data. However, the consequences of access control configuration failures by system administrators in a large organization are more severe, as they can impact the entire infrastructure of the organization and its customers \cite{bauer2009real, barrett2004field, botta2007towards}. System administrators or "sysadmins" typically have access to critical data and resources of the organization such as user data, financial data, etc. \cite{johnson2010optimizing}. If they do not properly restrict access to those critical data, a third party from outside of the organization or even from the inside of the organization \cite{bauer2009real} will be able to manipulate them, causing financial and reputation damage \cite{bauer2009real}. Société Générale Bank faced such an incident in 2008 due to poorly configured access control policies in their authorization system, reporting the largest trading loss in banking history \cite{bauer2009real}. In the incident, the Société Générale Bank lost \$7.2 billion over three days of trading due to unauthorized trades by an employee \cite{bauer2009real}. That employee was recently promoted to a junior trader from a compliance position where he monitored trading. However, the system administrator did not properly re-configured the access privileges by revoking the permissions related to the previous role of that employee. As a result, he was able to use those previous privileges together with his knowledge of trading gained when he worked in the compliance position to engage in unauthorized trades, causing a significant financial loss (\$7.2 billion) to the bank \cite{bauer2009real}. 

% Therefore, in order to avoid such losses, administrators should be provided with effective tools \cite{botta2007towards}. Therefore, by acknowledging the severity of the damage, we conduct this study by focusing on tools and techniques utilized to avoid administrator-centered policy configuration and generation failures.




\section{Related Work}
\label{sec:related_works}
% \textbf{I FIND A BIT BIZARRE THAT SECTION TWO IS ACTUALLY A RELATED WORK SECTION. I THINK WE SHOULD MOVE SECTION 3 UP WHERE WE EXPLAIN HOW THIS SOK WAS PLANNED AND CONDUCTED. }

Previous research initially attempted to solve access control failures by guiding the system administrator to write policies via graphical user interfaces (GUIs) \cite{reeder2008expandable, morisset2018visabac}. An example of such interfaces would be the template-based policy authoring interface shown in Fig. \ref{fig:gui_tools}(d) \cite{johnson2010usable}. It provides pre-defined templates such as \texttt{\{Subject\} can \{Action\} \{Target\}} to write policies by choosing suitable policy components for the placeholders denoted by "\{\}" \cite{johnson2010usable, johnson2010optimizing}. This interface guides administrators by pointing out what the necessary policy components are (i.e., subject, action, and target) and in what way those components should be organized in the policy \cite{johnson2010usable}. Therefore, by following the provided template, administrators can avoid incorrect access control policies (i.e., policies containing wrong policy components in wrong placeholders) and incomplete 
access control policies (i.e., policies without necessary policy components). However, the limitations of the existing tools make policy configuration difficult for administrators ~\cite{inglesant2008expressions}. For example, sometimes, their intended policies cannot be easily written according to the provided policy template. Assume that the administrator has to configure a complex policy like \emph{"Bob is allowed to access the computer "A" if the time is between 9 a.m. and 5 p.m."}, using the mentioned template-based authoring interface. However, if the interface does not support conditions 
% such as \emph{"if the time is between 9 a.m. and 5 p.m."}. Therefore, 
as a workaround, the administrator might neglect the condition entirely and generate a policy that allows Bob to access the computer at all times, without any restrictions. These situations may result in access control failures leading to data breaches \cite{reeder2007usability, maxion2005improving, brostoff2005r}. Therefore, to avoid such negative consequences due to access control failures, it is imperative to understand where these limitations are in policy authoring and visualization interfaces and provide solutions. With that in mind, previous literature that proposed such tools evaluated their interfaces individually and pointed out the limitations via user studies \cite{reeder2008expandable, karat2006evaluating, vaniea2008evaluating, stepien2009non, bertard2020using}. For instance, in the conducted user study, Johnson et al. also observed that their templates are overly flexible, allowing the policy author to fill the placeholder with any policy element without any restriction (i.e., \texttt{\{Subject\}} placeholder accepts any subject element in the organization even if it should not be allowed to perform the \texttt{\{Action\}} on the \texttt{\{Target\}}) \cite{johnson2010usable}. Such limitations cause access control failures resulting in data breaches that have the potential for severe financial \cite{bauer2009real} and reputation damages \cite{Heiligenstein_2023} of the organization. Therefore, Deleat et al. have introduced a framework in their survey to compare the usability of system configuration tools to decide what tool is best suited for a particular system configuration task \cite{delaet2010survey}. However, since they focus on system configuration tools, they only mentioned the effect of their framework on access control policy configuration briefly \cite{delaet2010survey}. In contrast to Deleat's work, Paci et al. also briefly discuss the usability and transparency of access control configuration interfaces such as access matrices \cite{lampson1974protection}, in their systematic literature review \cite{paci2018survey}. However, they only focused on the end user's perspective of access control configuration in community-centered collaborative systems such as Facebook. Therefore, it is important to have a holistic idea about the common problems of those graphical access control configuration tools as a whole from the administrator's perspective, to develop usable policy authoring and visualization tools for administrators. Therefore, we conducted this SLR by considering all such tools we identified in the extracted literature to highlight their limitations.  

However, even if graphical policy authoring interfaces guide the administrator to write correct and complete policies, those tools still fail to provide a complete solution to access control failures. Because failures can still occur due to human errors driven by mental conditions such as stress and fatigue of system administrators \cite{palmer_2021}. For example, in the mentioned template-based policy authoring interface, the administrator has to choose and apply the correct policy components to the correct placeholders manually. Also, it has to be done repetitively if there are many policies in the organization. This repetitive process is considered as an overhead by the security experts, which can lead to stress and fatigue \cite{narouei2017identification,botta2007towards, palmer_2021}. If administrators are stressed and fatigued, the probability of making a mistake in policy configuration, such as allowing an unauthorized person to access the computer instead of Bob, is high \cite{botta2007towards, reeves2021encouraging, palmer_2021}. Therefore, as a solution, previous research also suggested removing the human factor (i.e., the administrator) entirely from policy generation by utilizing automated policy generation frameworks consisting of ML/NLP techniques \cite{shi2011controlled, xia2022automated}. However, those ML/NLP techniques employed in automated policy generation frameworks are not reliable enough to generate machine-executable policies without human supervision \cite{kaur2021human}. For example, ML models are often prone to false positives and false negatives. Therefore, if a generated policy with falsely identified policy components is applied to the access control system without being verified by an administrator, it causes security holes in the system. Those holes can open up a back door to hackers, resulting in data breaches. These kinds of limitations were also pointed out by one other published systematic mapping study \cite{ del2018systematic}. 
% Nobi et al. identified several reasons that make the machine learning-based policy configuration tools ineffective \cite{nobi2022machine}. For instance, they point out that the lack of "good" datasets hinders the performance of ML models, making them less reliable. Furthermore, by corroborating Nobi's findings, 
Alamo et al. pointed out why the existing NLP-based techniques are ineffective in policy analysis \cite{del2022systematic}. According to their findings \cite{del2022systematic}, neural network-based policy analysis techniques sometimes fail to identify privacy policies (i.e., low recall). At the same time, the traditional ML-based approaches tend to identify privacy policies falsely \cite{del2018systematic} (i.e., low precision). All the above findings support our claim that even if the automated solutions alleviate the administrator's overhead, they still are not reliable enough to operate without human involvement \cite{ del2022systematic}. 

Despite having these challenges in both the graphical policy authoring and visualization interfaces and automated policy generation frameworks, all the existing surveys/systematic literature reviews focus either on the usability of graphical policy configuration \cite{paci2018survey, delaet2010survey} or the reliability of automated policy generation \cite{del2018systematic}. Furthermore, none of them mainly focus on these challenges in access control policy configuration and generation from the system administrator's perspective.
% All of them were based on the fact that addressing the limitations of the automated policy generation process will resolve access control failures \cite{nobi2022machine, del2022systematic} no matter how the administrators interact with the process. 
Nevertheless, improving fully automated policy generation frameworks \cite{shi2011controlled, alohaly2018deep, alohaly2021hybrid, amato2013semantic, fatema2016semi, slankas2013access, heaps2021access, slankas2013accessid, brodie2006empirical, xia2022automated, alohaly2019automated, xiao2012automated, narouei2018automatic, narouei2015automatic, slankas2012classifying, singru2020efficient, vaniea2008evaluating, rosa2020parser, inglesant2008expressions, liu2017automated, narouei2017identification, ye2016identify, slankas2013implementing, perry2013modular, basile2010ontology, yang2021purext, slankas2014relation, narouei2017towards, alohaly2019towards, narouei2015towards, tanoli2018towards, zhu2021unstructured, brodie2005usable, shen2021using, abdelgawad2023synthesizing} alone will not effectively reduce access control failure, as it lacks the human administrator's expertise to verify the generated policies \cite{kaur2021human}. At the same time, improving graphical policy authoring and visualization tools \cite{stepien2009non,stepien2014non, bertard2020using, turner2017proposed, brostoff2005r, zurko1999user, johnson2010usable, johnson2010optimizing, maxion2005improving, cao2006intentional, reeder2007usability, reeder2008expandable, morisset2018visabac, reeder2011more, karat2006evaluating, morisset2018building} also will not mitigate access control failures as it induces accidental human errors due its manual and repetitive nature \cite{kaur2021human, narouei2017identification, narouei2017towards, nobi2022machine}. Therefore, while we agree the fact that both of those approaches should be improved by addressing their existing limitations, we further argue that the correct balance between manual and automated policy generation techniques will help develop more usable as well as reliable policy generation tools while reducing the administrator's overhead. For that, first, the limitations of graphical policy authoring and visualization tools (i.e., manual approach) and the limitations of NLP-based automated policy generation frameworks (i.e., automated approach) should be identified. Therefore, we conducted this SLR by focusing on both the graphical policy authoring and visualization tools and NLP-based policy generation frameworks to point out their limitations. Addressing those limitations will help improve those tools and frameworks further and develop more effective policy generation frameworks that leverage the automation capabilities of reliable NLP techniques as well as the administrator's expertise via a usable interface. Those frameworks will help improve the usability and reliability of access control policy generation, addressing the usability-security trade-off. 

% However, the security risk of over flexibility should also be avoided as we discussed in Section \ref{subsubsec: gui}.
% However, as we identified in Section \ref{subsubsec: gui}, over-flexibility also causes access control failures. Therefore, as solutions, providing default templates to support a wide range of access control policies and not allowing the administrator to create general templates that accept any value for a placeholder can be implemented \cite{nielsen2005ten}. 



\section{Intro}

\textcolor{blue}{On July 17, 2019, Capitol One, one of the largest credit card companies in the world, received an email with a link to a GitHub file, saying that there are leaked company data published in a GitHub account \cite{Siegel_2019}. Upon receiving that email, Capitol One examined the file and found that it contains 120,000 Social Security numbers and 77,000 bank account numbers extracted from roughly 100 million of their credit card applications \cite{Siegel_2019}. The investigation tigations revealed those data were leaked by a hacker known as "eratic" by exploiting a misconfiguration in Capitol One's firewall that allowed commands to reach and be executed by a remote server. To steal that personal information, first, the hacker obtained credentials for one of the accounts of the company and, in turn, gained access to certain Capitol One folders. Once gaining access to those folders, the hacker was able to copy data from those folders and later published them in GitHub, causing a severe data breach \cite{Siegel_2019}.} 
% These kinds of data breaches raise two basic questions: Why those data breaches are happening? And due to whose fault?} 

\textcolor{blue}{One of the main reasons for such data breaches is access control failures that allow unauthorized parties, such as hackers, to access the organization's network and then allow them to access the private information of the organization and its customers by exploiting vulnerabilities in the organization's authorization system \cite{bauer2009real, reeder2008expandable, maxion2005improving}. Therefore, even if the organization's network is safe, if access to its private information is not properly restricted by the system administrator, defining who can access the information and under what circumstances, the chance for a data breach is high \cite{bauer2009real}. For example, it has been found that, most access control failures occur when employees or former employees in the organization are able to use their legitimate credentials to commit crimes (e.g., data leaks) because they have been given inappropriate access to the system or they were not revoked in a timely manner by the system administrator \cite{bauer2009real}.}


% For instance, statistical NLP/ML techniques were used in most of the existing automated policy generation frameworks to identify policies from natural language policy requirement documents and extract their policy components \cite{slankas2014relation, xia2022automated, heaps2021access, narouei2015automatic, alohaly2019towards}. However, since those techniques were less accurate, sometimes they might not identify natural language policies or extract policy components correctly \cite{heaps2021access}. As a result, machine-executable policies generated from those incorrectly extracted policy components will also be incorrect. Suppose those incorrect policies are applied to the authorization system without being verified by a system administrator. In that case, there is a chance that the wrong user gains access to the wrong resource. These unexpected behaviors of the automated policy generation frameworks (i.e., automation surprise \cite{kaur2021human}) cause access control failures leading to data breaches. 


% Consequently, such conditions affect the administrator's decision-making ability which leads to mistakes when generating or configuring access control policies \cite{reeves2021encouraging}. For instance, when the administrator is fatigued, they might overlook important permissions and grant unauthorized access to resources causing access control failures \cite{xu2017system}. 

% Therefore, it is important to identify the common challenges of such tools as a whole to get an overall idea of their usability. With that in mind, Deleat et al. have introduced a framework in their survey to decide what tool is best suited for a secure system configuration task based on their usability \cite{delaet2010survey}. However, since they focus on system configuration tools, they did not specifically focus on access control configuration tools \cite{delaet2010survey}. Furthermore, Paci et al. also briefly discuss the usability of access control configuration tools such as access matrices \cite{lampson1974protection} in their systematic literature review conducted focusing on access control in community-centered collaborative systems such as Facebook \cite{paci2018survey}. However, they only focused on the usability of such tools from the end user's perspective. 
% Therefore, it is important to have a holistic idea about the common limitations of graphical access control configuration tools as a whole, from the administrator's perspective, to develop usable tools for administrators to avoid administrator-centered access control failures. Therefore, we conducted this SLR by considering such tools we identified in the extracted literature to highlight their limitations from the administrator's perspective. 
